Nearly Tight Bounds on Testing of Metric Properties

Given a non-negative $n \times n$ matrix viewed as a set of distances between $n$ points, we consider the property testing problem of deciding if it is a metric. We also consider the same problem for two special classes of metrics, tree metrics and ultrametrics. For general metrics, our paper is the first to consider these questions. We prove an upper bound of $O(n^{2/3}/\epsilon^{4/3})$ on the query complexity for this problem. Our algorithm is simple, but the analysis requires great care in bounding the variance on the number of violating triangles in a sample. When $\epsilon$ is a slowly decreasing function of $n$ (rather than a constant, as is standard), we prove a lower bound of matching dependence on $n$ of $\Omega (n^{2/3})$, ruling out any property testers with $o(n^{2/3})$ query complexity unless their dependence on $1/\epsilon$ is super-polynomial. Next, we turn to tree metrics and ultrametrics. While there were known upper and lower bounds, we considerably improve these bounds showing essentially tight bounds of $\tilde{O}(1/\epsilon )$ on the sample complexity. We also show a lower bound of $\Omega ( 1/\epsilon^{4/3} )$ on the query complexity. Our upper bounds are derived by doing a more careful analysis of a natural, simple algorithm. For the lower bounds, we construct distributions on NO instances, where it is hard to find a witness showing that these are not ultrametrics.

==> extra-things.tex <==
It remains to show that $\tilde{M}\in\calP^T$, which we do by considering an arbitrary quadruple $i, j, k,l \in [n]$, and show that it does not form a violation in $\tilde{M}$. First, by same reason as in Lemma~\ref{lem:large-EC-ODC}, a simple case occurs when at least one of four $i,j,k$ or $l$ had been inconsistent with $S$. A second easy case occurs when all $i,j,k,l \in S$.

    Now, we go into a case analysis for the remaining cases.
    \begin{itemize}
        \item Suppose $i,j,k\in S$ and $l\in[n]\setminus S$ is consistent. Then by definition of consistency, $S\cup\{l\}$ is consistent; moreover, the distances from $l$ to $S$ remain the same in $\tilde{M}$ as in $M$. Thus, $\{i,j,k,l\}$ are not violating in $\tilde{M}$.
        \item Suppose $i,j\in S$ and $k,l\in[n]\setminus S$ are consistent. Since $k,l$ are consistent, for below cases, we have $\tilde{M}(k,u)=M(k,u)$ and $\tilde{M}(l,u)=M(l,u)$ for all $u\in S$. We go to a case analysis on whether $k,l$ are in the same part or not.
        \begin{itemize}
            \item Suppose $k,l$ are in the same part $P$. If $P$ is Easy or Active, $\tilde{M}(k,l)=M(u,k)+M(u,l)-\min_{k',l'\in P_\ell}\{M(u,k')+M(u,l')\}$ for some $u\in S$. Suppose the minimum is taken on $k',l'\in P$. By the definition of $k,l$ falling into the same part, $M(k,i)+M(l,j)=M(k,j)+M(l,i)$. Moreovoer, $M(i,j)\leq M(i,k')+M(j,k')=(M(k',i)+M(l',j)+M(k',j)+M(l',i))/2$ by triangle inequality as $k',l'$ are consistent. Thus, $M(i,j)\leq M(i,k')+M(j,l')$ which is equivalent to $M(i,j)+M(u,k)+M(u,l)\leq M(i,k')+M(u,k)+M(j,l')+M(u,l)=M(i,k)+M(u,k')+M(j,l)+M(u,l')$. This leads to $\tM(k,l)+M(i,j)\leq M(i,k)+M(j,l)=\tM(k,j)+\tM(l,i)$, indicating that the quadruple is not violating in $\tM$. If $P$ is Versatile, $\tM(k,l)=M^\ast_P(k,l)$ and by definition of $M^\ast_P$, the distances $M(i,j),M(i,k),M(i,l),M(j,k),M(j,l),M^\ast_P(k,l)$ obey the four-point-condition. Thus, the quadruple is not violating in $\tM$. Notice that this argument shows that, whenever we have the two indices in the same part and two other indices in $S$, out of the three matchings, the one that matches the two indices in the same part together and the two indices in $S$ together is no larger than the other two matchings in $\tM$.
            \item Suppose $k,l$ are in different parts $P,P'$ respectively.  We go into two cases for whether $(k,l)$ is in $\SC(M,S)$. If $(k,l)\notin \SC(M,S)$, then $\tM(k,l)=M(k,l)$. Moreover, for all pairs $(u,v) \in S^2,$ $M(k,l)+M(u,v)=\max\{M(k,u)+M(l,v),M(k,v)+M(l,u)\}$. Thus, $\{i,j,k,l\}$ is not violating in $\tilde{M}$. Suppose $(k,l)\in \SC(M,S)$. Then, there exists some $(u,v)$ such that $M(k,u)+M(l,v)\neq M(k,v)+M(l,u)$ and $\tM(k,l)=\max\{M(k,u)+M(l,v), M(k,v)+M(l,u)\}-M(u,v)$. Without loss of generality, after re-naming the indices, assume $M(k,u)+M(l,v)< M(k,v)+M(l,u)$. Then, $\tM(k,l)+M(u,v)=M(k,v)+M(l,u)$. Since the quadruples $\{i,u,v,k\}$ and $\{j,u,v,k\}$ are non-violating as they contain three indices from $S$, one of the following must hold, for each quadruple, the max two matchings are equal. Below we give the analysis for one case, $M(i,v)+M(u,k)=M(i,k)+M(u,v)$ and $M(j,v)+M(u,k)=M(j,k)+M(u,v)$, and the rest cases follow the similar argument. Then, as $\{i,j,v,l\}$ is not violating, we either have $M(j,v)+M(l,i)=\max\{M(i,j)+M(v,l),M(i,v)+M(l,j)\}$ or $M(i,j)+M(v,l)=M(i,v)+M(l,j)\geq M(j,v)+M(l,i)$. Suppose it is the former case. Then $M(j,v)+M(l,i)+M(u,k)-M(u,v)=\max\{M(i,j)+M(v,l)+M(u,k)-M(u,v),M(i,v)+M(l,j)+M(u,k)-M(u,v)\}.$ The first term, $M(i,j)+M(v,l)+M(u,k)-M(u,v)$, is less than $M(i,j)+M(k,v)+M(l,u)-M(u,v)=M(i,j)+\tM(k,l)$ by assumption $M(k,u)+M(l,v)<M(k,v)+M(l,u)$. The second term, $M(i,v)+M(l,j)+M(u,k)-M(u,v)=M(k,i)+M(l,j)$ by assumption $M(i,v)+M(u,k)=M(i,k)+M(u,v).$ Lastly, $M(j,v)+M(l,i)+M(u,k)-M(u,v)=M(k,j)+M(l,i)$ by assumption $M(j,v)+M(u,k)=M(j,k)+M(u,v)$. Therefore, the quadruple $\{i,j,k,l\}$ obey the four-point condition in $\tM$.
        \end{itemize}
        \item Suppose $i\in S$ and $j,k,l\in[n]\setminus S$ are consistent.
        \begin{itemize}
            \item If $j,k,l\in[n]\setminus S$ are in the same $P$ for $P$ being Active or Easy, then for some $u\in S$, their pairwise distances are set to $\tM(j,k)=M(u,j)+M(u,k)-\min_{j',k'\in P}\{M(u,j')+M(u,k')\},$ $\tM(j,l)=M(u,j)+M(u,l)-\min_{j',k'\in P}\{M(u,j')+M(u,k')\},$ and $\tM(k,l)=M(u,k)+M(u,l)-\min_{j',k'\in P}\{M(u,j')+M(u,k')\}.$ To show the quadruple is non-violating is equivalent to showing the maximum of $\{M(u,j)+M(u,k)+M(i,l),M(u,j)+M(u,l)+M(i,k),M(u,k)+M(u,l)+M(i,j)\}$ is not unique. Since $\{j,k,l\}$ are in the same part, $M(u,k)+M(i,l)=M(i,k)+M(u,l)$, so the first and second terms are the same. By same argument, the second and the third term are the same. Now consider $P$ being a Versatile Part. Then, $\{i,j,k,l\}$ is not violating exactly because of the definition of $\tM(j,k)=M^\ast_P(j,k),\tM(j,l)=M^\ast_P(j,l),\tM(k,l)=M^\ast_P(k,l)$ and matrix $M^\ast_P$ incur a tree metric together with $M$.
            \item If $j,k$ are in the same part $P$ and $l$ is in a different part $P'$. Then there exists a pair $(u,v)\in\SEP(k,l)\subset S$ such that $M(k,u)+M(v,l)\neq M(k,v)+M(l,u).$ Without loss of generality, assume $M(k,u)+M(v,l)> M(k,v)+M(l,u)$. Since $\{k,l,u,v\}$ is not violating as the quadruple contain two indices in $S$ by above argument, $\tM(k,l)+\tM(u,v)=\max\{\tM(k,u)+\tM(v,l),\tM(k,v)+\tM(l,u)\}=\tM(k,u)+\tM(v,l)=M(k,u)+M(v,l)$. Moreover, since $j,k$ are in the same part, we must have $M(k,u)-M(k,v)=M(j,u)-M(j,v).$ Since $M(k,u)-M(k,v)>M(l,u)-M(v,l),$ we also have $M(j,u)-M(j,v)>M(l,u)-M(v,l)$ which leads to $M(j,u)+M(v,l)>M(l,u)+M(j,v).$ Now, since $\{u,v,j,l\}$ is not violating, we have $\tM(j,l)+\tM(u,v)=\max\{\tM(j,u)+\tM(v,l),\tM(j,v)+\tM(u,l)\}=M(j,u)+M(v,l).$ In summary, we have the equations $\tM(k,l)=M(k,u)+M(v,l)-M(u,v)$ and $\tM(j,l)=M(j,u)+M(v,l)-M(u,v)$. By argument above in the two indices in the same part and two indices in $S$ case, out of the three matchings, the one that matches the two indices in the same part together and the two indices in $S$ together is no larger than the other two matching in $\tM$. These lead to $\tM(k,l)+\tM(i,j)=M(k,u)+M(v,l)-M(u,v)+M(i,j)=M(k,i)+M(j,u)+M(v,l)-M(u,v)=\tM(j,l)+M(k,i)=\tM(j,l)+\tM(k,i)$. Moreover, $\tM(j,k)+\tM(i,l)\leq \tM(k,l)+\tM(i,j)$. Thus, the quadruple is not violating.
            \item Suppose $j,k,l$ are in three different parts. Consider an arbitrary $u\in S$. We want to show that the maximum in the set $\{\tM(i,j)+\tM(k,l),\tM(i,k)+\tM(j,l),\tM(i,l)+\tM(j,k)\}$ is not unique. Consider the quadruples $\{i,u,k,l\}$,$\{i,u,j,k\}$,$\{i,u,j,l\}$. They are not violating in $\tM$ because each contains two indices in $S$. We go into case analysis on the combinations of whether $\tM(k,l)+\tM(i,u)$ is the max among the three matchings in $\{i,u,k,l\}$, whether $\tM(j,k)+\tM(i,u)$ is the max among $\{i,u,j,k\}$, and whether $\tM(j,l)+\tM(i,u)$ is the max among $\{i,u,j,l\}$. 
            \begin{itemize}
                \item Suppose $\tM(k,l)+\tM(i,u)$ is the max among $\{i,u,k,l\}$ and $\tM(j,k)+\tM(i,u)$ is smaller than the max among $\{i,u,j,k\}$ and $\tM(j,l)+\tM(i,u)$ is smaller than the max among $\{i,u,j,l\}$. Then $\tM(i,j)+\tM(u,k)=\tM(i,k)+\tM(u,j)$ and $\tM(i,j)+\tM(u,l)=\tM(i,l)+\tM(u,j)$.
            \end{itemize}

        
        \end{itemize}
        \item Suppose $i,j,k,l\in[n]\setminus S$ are consistent. If all four are in the same part, then by same argument as before, every quadruple inside Easy Part or Versatile Par or Active Part is not violating. 
    \end{itemize}




    
\subsection{Our Contributions}

We provide three efficient algorithms for testing $\epsilon$-farness for general metric property, ultrametric property, and tree metric property. Along with the testing algorithms, we also construct adversarial objects to show that our tester almost match the lower bound for testing. Quantitatively, we have the following results.
\begin{itemize}

    \item \textbf{General metric}
    \begin{itemize}   
    \item  
    It is possible to test whether a matrix in $M\in\mathbb{R}^{n\times n}$ is a metric $\mathcal{P}$ on $n$ points, or far from being a metric with $O(n^{2/3}/\epsilon^2)$ queries.
    \item We provide constructions of distance matrices to show that non-adaptive algorithms allowed to have two-sided error must make $\Omega (n^{2/3}/\epsilon^{2/3})$ queries to distinguish metrics from matrices that are $\epsilon$-far from being a metric, for $\epsilon\leq n^{-\nu(n)}$ where $\nu(n)$ is a very slowly decreasing function.
    \end{itemize}
    \item \textbf{Ultrametric}
    \begin{itemize}
       
    \item It is possible to test whether a matrix is an ultrametric on $n$ points or $\epsilon$-far with $\tilde{O} (1/\epsilon)$ sampled points, which corresponds to $\tilde{O}(1/\epsilon^2)$ pairwise queries.
    \item Any testing algorithm must make $\Omega(1/\epsilon^{4/3})$ queries to distinguish ultrametrics from matrices that are $\epsilon$-far from being an ultrametric. In terms of sample size, any testing algorithm must sample $\Omega(1/\epsilon)$ points to distinguish ultrametrics from matrices that are $\epsilon$-far from being an ultrametric.
    \end{itemize}
    
    \item \textbf{Tree metric}
    \begin{itemize}
        \item 
    It is possible to test whether a matrix is a tree metric on $n$ points or $\epsilon$-far with $\tilde{O} (1/\epsilon)$ sampled points, which corresponds to $\tilde{O}(1/\epsilon^2)$ pairwise queries.
    \item Any testing algorithm must make $\Omega(1/\epsilon^{4/3})$ queries to distinguish ultrametrics from matrices that are $\epsilon$-far from being an ultrametric. In terms of sample size, any testing algorithm must sample $\Omega(1/\epsilon)$ points to distinguish ultrametrics from matrices that are $\epsilon$-far from being an ultrametric.
    \end{itemize}
    
\end{itemize}

\subsection{Outline}
In section~\ref{sec:general}, we provide a testing algorithm for general metric and construct two matrices to show the hardness for testing for both one-sided and two-sided error testing algorithms. In section~\ref{sec:ultra}, we provide an algorithm for testing ultrametric. In section~\ref{sec:tree}, we modify the tester for ultrametric and use it for tree metric testing. Lastly, we construct hard case instances to show the sample complexity lower bound for both ultrametric and tree metric testing in section~\ref{sec:samplelb} and query complexity lower bound in section~\ref{sec:querylb}.




\section{Preliminaries}
In the study of property testing, suppose $\mathcal{S}$ is the universe of all objects of our concern, then a property $\mathcal{P}$ is a subset of $\mathcal{S}$ which contains all objects satisfying some conditions. An object has the property $\mathcal{P}$ if it is inside the subset $\mathcal{P}$. Moreover, an object $O$ is far from the property $\mathcal{P}$ if for any object $O'\in\mathcal{P},$ the distance between $O$ and $O'$ is at least some threshold under certain appropriately defined quantitative distance measure.

In this paper, the objects are distance matrices in $\mathbb{R}^{n\times n}$ and the distance measure between matrices is $\ell$-0 distance. We define a matrix to be $\epsilon$-far from a property if at least $\epsilon$ fraction of its entries need to be modified for it to be some matrix possessing the property.
\begin{definition}[$\epsilon$-farness]
    A distance matrix $M\in\mathbb{R}^{n\times n}$ is $\epsilon$-far from a metric property $\mathcal{P}$ if, for any matrix $M'\in\mathcal{P}$, $|M-M'|_0\geq \epsilon n^2$. That is, $M$ and $M'$ differ on at least $\epsilon n^2$ entries.
\end{definition}



\section{Sample Complexity Lower Bound For Tree and Ultrametric Testing}\label{sec:samplelb}

Both the ultrametric testing algorithm and the tree metric testing algorithm sample $\tilde{O}(1/\epsilon)$ points and make pair-wise query. We show that this sample complexity is almost tight: below is a bad case instance which is $\epsilon$-far from an ultrametric or a tree metric. Moreover, any one-sided error testing algorithm must sample at least $\Omega(1/\epsilon)$ points from the matrix to detect a corruption.

The adversarial distance matrix is constructed as follows. Suppose the $n$ points are divided into two groups, $G=\{x_1,x_2,...,x_r\},$ $B=\{y_1,...,y_s\}$, where $|G|=r=n-\epsilon n$ stands for the good points and $|B|=s=\epsilon n$ stands for the bad points. In the corrupted distance metric, $M(x_i,x_j)=2n,M(x_i,y_j)=2n+i,M(y_i,y_j)=2n$. Since $i\leq r<n$, any three such distances obey triangle inequality, so $M$ is indeed a metric.

A metric is an ultrametric if and only if for every triple $(a,b,c),$ the two largest distances in $d(a,b),d(a,c),d(b,c)$ equal. $M$, according to the above construction, is not an ultrametric because triples of the form $(x_i,x_j,y_l)$ do not obey this definition. On the other hand, this is an if and only if statement: triples that violate the ultrametric requirements are exactly of the form $(x_i,x_j,y_l)$. Therefore, to detect a corruption, any algorithm must hit a point in the bad set, $B$. Since $B$ contains $\epsilon$ fraction of the total points, any algorithm needs to sample at least $\Omega(1/\epsilon)$ points to detect a corruption.

As for tree metric constraints, tuples of the form $(x_i,x_j,x_k,y_l)$ violate the four-point condition. One can also check that tuples that violate the four-point condition are exactly of this form. By the same argument as above, any testing algorithm needs to sample at least $\Omega(1/\epsilon)$ points to hit a point in the bad set $B$ and, in consequence, detect a corruption.

\begin{lemma}
    The metric $M$ is $\Omega(\epsilon)$-far from an ultrametric and $\Omega(\epsilon)$-far from a tree metric. 
\end{lemma}
\begin{proof}
First, if we modify all $M(x_i,y_j)$ to be $2n$, then the new metric is an ultrametric (and so also a tree metric) since it represents a star-shaped tree. There are $(n-\epsilon n)\epsilon n\sim \epsilon n^2$ many such entries.

On the other hand, all triples of the form $(x_i,x_j,y_l)$ violate the ultrametric property, since $M(x_i,x_j)=2n<M(x_i,y_l)=2n+i<M(x_j,y_l)=2n+j$ assuming, without loss of generality, that $i<j.$ There are ${n-\epsilon n\choose 2}\epsilon n\sim\Omega(\epsilon n^3)$ such triples. A modification of any $M(x_i,y_l)$ entry corrects at most $n-\epsilon n\sim\Omega(n)$ such triples; a modification of any $M(x_i,x_j)$ entry corrects at most $\epsilon n$ such triples. Since at least $\Omega(\epsilon n^3)$ triples need to be corrected, we need to modify at least $\Omega(\epsilon n^2)$ many entries.

Similarly, all tuples of the form $(x_i,x_j,x_k,y_l)$ violate the four-point condition. There are $\Omega(\epsilon n^4)$ such tuples. The modification of $M(x_i,y_l)$ entry corrects at most $\Omega(n^2)$ such tuples, and the modification of $M(x_i,x_j)$ entry corrects at most $\Omega(\epsilon n^2)$ such tuples. Therefore, we need to modify at least $\Omega(\epsilon n^2)$ entries to correct $\Omega(\epsilon n^4)$ such tuples.
\end{proof}

\section{Query Complexity Lower Bound For Tree and Ultrametric Testing}\label{sec:querylb}
The bad case instance constructed in the above section shows that gives a lower bound on the sample complexity. Any testing algorithm needs to sample at least $\Omega(1/\epsilon)$ points before detecting a violation. However, the query complexity, or the number of entries a tester needs to sample, for testing this adversarial matrix has only the trivial lower bound $\Omega(1/\epsilon)$.

Below, we construct a distance matrix which is $\epsilon$-far from tree metric (so it is also $\epsilon$-far from ultrametric) and any algorithm has to sample $\Omega(1/\epsilon^{2/3})$ points before detecting a violation to the tree metric property. Moreover, the algorithm needs to make pairwise clique like query before detecting a violation. This suggests that the query complexity is bounded below by $\Omega(1/\epsilon^{4/3})$.

We first demonstrate the idea for constructing this hard case instance. Recall that for a matrix to be a tree metric, any four-point-tuple needs to obey the four-point condition. Namely, the larger two matchings have the same value. Suppose the adversary starts with some tree metric $M$. Consider points $i,j,k,l,$ and without loss of generality, suppose the value of the matching $M(i,j)+M(k,l)$ is no larger than the other two matchings $M(i,k)+M(j,l)=M(i,l)+M(j,k)$. The adversary toggles with the shorter distance $M(i,j)$ (or $M(k,l)$), so that the four-point condition still holds for $i,j,k,l$. This adversarial change is un-noticable unless the distance $M(i,j)$ (or $M(k,l)$) was among the larger two matchings for some other 4-point tuple $i,j,x,y$ (or $k,l,x,y$). Thus, the idea for the adversary is to corrupt the entries that correspond to ``short distances" in the original tree metric, so that only an even shorter pair is chosen can a tester notice the violation the 4-point condition.

Thus, we choose to corrupt $1/\alpha$ small clusters of size $\alpha n$ on a tree metric. A small cluster, in this context, is a set of points $C$ which satisfies $u,v\in C\Rightarrow M(u,v)<M(u,w)$ and $M(u,v)<M(v,w)$ for any $w\notin C$. In this case, if for a four-point tuple, no more than 2 points are drawn from the same cluster, then the larger two sums are the same so a tester cannot notice any violation.

We now give a concrete lower bound construction. Consider an $n\times n$ distance matrix defined as following.
\[
\renewcommand\arraystretch{1.3}
D=\mleft[
\begin{array}{c|c|c|c|c}
  D_1 & \ast &\ast &\cdots &\ast\\
  \hline
  \ast & D_2 & \ast &\cdots &\ast\\
  \hline
  \ast & \ast & D_3 &\cdots &\ast\\
  \hline
  \vdots & \vdots & \vdots &\ddots &\vdots\\
  \hline
  \ast & \ast & \ast &\cdots &D_k\\
\end{array}
\mright]
\]
where $\ast$ is a $q\times q$ block matrix such that each entry equals $10^q$; $D_i$ is a $q\times q$ block matrix of the form
\[
\renewcommand\arraystretch{1.3}
D_i=\mleft[
\begin{array}{ccccccc}
  0 & 1 &10 &100&1000&\cdots &10^{q-2}\\
  1 & 0 & 20&200&2000&\cdots &2\cdot10^{q-2}\\
  10 & 20 & 0&300&3000&\cdots &3\cdot10^{q-2}\\
  100 & 200 & 300&0&4000&\cdots &4\cdot10^{q-2}\\
  \vdots & \vdots & \vdots & \vdots& \ddots&\ddots &\vdots\\
  10^{q-2} & 2\cdot 10^{q-2} & 3\cdot 10^{q-2}&4\cdot10^{q-2}&5\cdot10^{q-2}&\cdots &q\cdot10^{q-2}\\
\end{array}
\mright].
\]
That is, a symmetric matrix with the $(i,j)^{th}$ entry being $D(i,j)=i\cdot 10^{j-2}$ for $i<j$, and zeros on the diagonal. We claim that $D_i$ is $\Omega(q^2)$ far from a tree metric. To see this, assume we have sampled $i<j<k<l$ four points in $D_i$. According to the distance matrix, we must have 
\begin{align*}
&D(k,l)+D(i,j)=k\cdot 10^{l-2}+i\cdot 10^{j-2}
\
\\>&D(j,l)+D(i,k)=j\cdot 10^{l-2}+i\cdot 10^{k-2}
\\>&D(i,l)+D(j,k)=i\cdot 10^{l-2}+j\cdot 10^{k-2}.
\end{align*}
This suggests the four-point condition is violated for all four point tuples. Thus, to modify $D_i$ to a proper tree metric, at least one of the 6 entries must be corrected for any four point tuples. There are ${q\choose 4}$ four point tuples and each $(i,j)$ pair is involved in ${q\choose2}$ four point tuples. Thus, at least ${{q\choose 4}}/{{q\choose2}}=\Omega(q^2)$ entries must be corrected.

This claim implies that at least $\Omega(q^2\cdot(n/q))$ entries of $D$ have to be modified for $D$ to become a tree metric. We take $q=\lfloor \epsilon n\rfloor$, then $D$ is $\epsilon$-far from a tree metric.

Now, straightforwardly, points $i,j$ belong to the same ``small cluster" if entry $(i,j)$ fall into some $D_i$. Notice that if for a four point tuple $\{i,j,k,l\}$, no three points fall into the same small cluster, then the four point criterion is not violated. If no more than three points fall into the same small cluster, then at least 4 of the entries among $D(i,j),D(i,k),D(i,l),D(j,k),D(j,l),D(k,l)$ fall into the $\ast$ block matrices. Thus, at least four distances equal $10\cdot q$ and the remaining distances are strictly less than $10\cdot q$, so the four point condition follows.

Suppose the testing algorithm picks $n'$ points uniformly at random. The algorithm only recognizes an error if at least three of the $n'$ points fall into the same cluster. Suppose $X_{i,j,k}$ is an indicator variable for whether points $i,j,k$ belong to the same cluster for all three tuples. Then, $\mathbb{E}[X_{i,j,k}]=\Omega(\epsilon^2).$ There are $\Omega(n'^3)$ 3-tuples formed in the sample set, so the expected number of 3-tuples that fall into the same cluster is $\Omega(\epsilon^2n'^3),$ which is greater than 1 if $n'=\Omega(1/\epsilon^{2/3})$ samples are selected. 

Now, we switch gear to analyze the query complexity. Suppose an testing algorithm samples $n'$ at random and chooses to query the distance between some selected pairs. It is equivalent to a graph on $n'$ vertices where two vertices are adjacent if and only if their distance is being queried. If, for any cluster, the subgraph induced by all vertices in that cluster does not contain any cycle, then the algorithm cannot detect a violation to the four-point condition. This is because, the only 4-tuples that violate the four-point condition in $D$ are those who have at least three points in the same cluster. Since the algorithm have not queried the pairwise distance between these three points, four-point test cannot be applied on the tuple.

Therefore, the situation is equivalent to making queries on a graph with $n'$ vertices; a tester detects a violation only when edges of some cycle in the graph all belong to a small cluster as defined above. We call the cycle ``survived" in this situation. For a $k$-cycle, all edges belong to the same cluster with probability $\epsilon^{k-1}.$ Hence, the expected number of survived cycles is $$\sum_{k=3}^\infty\epsilon^{k-1}\cdot(\text{number of cycles with length }k),$$ and an algorithm aims to pick a query graph structure to maximize this quantity. The following lemma shows that among the $n'$ sampled, making a ``clique-like" query graph structure is optimal for a testing algorithm.

\begin{lemma}
Suppose the adversary uses the above distance matrix $D$. A testing algorithm is allowed to pick $m$ pairs of points and query the distance, and the number of points $n'$ involved in the queries is chosen under the algorithm's discreet. To maximize the expected number of survived simple cycles as defined above, the algorithm should select $n'$ points such that ${n'\choose2}\geq m>{n'-1\choose 2}$ and make $m$ queries on the graph with these points. That is, a graph with $m$ edges that is closest to a clique maximizes the quantity.
\end{lemma}
\begin{proof}
Given the choice to make $m$ queries, an algorithm wants to maximize the expectation $\sum_{k=3}^\infty\epsilon^{k-1}\cdot(\#\text{ of cycles with length }k)$. Let $n'$ be an integer defined as in the statement. We start with an arbitrary graph $G$ with $l>n'$ vertices and $m$ edges, and show that $G$ can be modified to $G'$ with strictly less vertices such that the quantity is larger. This ``graph modification" is done by ``merging" two vertices and adding edges between previously non-adjacent vertices.

First, we modify $G$ such that its diameter is at most 2. Suppose initially the diameter of $G$ is larger than 2. Then, there exists a pair of vertices $(x,y)$ such that the neighbor of $x$, $N_x$, is disjoint from that of $y$, $N_y$. We ``merge" $(x,y)$ to obtain a new vertex $z$, such that previously existing edges of the form $(v_1,x),(v_2,y)$ become $(v_1,z),(v_2,z)$. This action only increases the objective quantity: 
\begin{itemize}
    \item Any cycle that do not contain $x,y$ still remains;
    \item Any cycle that only contains one of $x,y$ still remains;
    \item Suppose cycle $C$ contains both $x,y$. Then it must be of the form $x\rightarrow v_1\rightarrow\cdots\rightarrow v_i\rightarrow y\rightarrow u_1\rightarrow \cdots\rightarrow u_j\rightarrow x,$ where $v_1\neq v_i$, $u_1\neq u_j$. Thus, merging $x,y$ gives two new cycles of strictly less lengths.
\end{itemize}

Now, suppose that $G$ is a graph with $l$ vertices with diameter at most 2. Since $l>n'$ where integer $n'$ satisfies ${n'\choose 2}\geq m$, we must have that at least ${l\choose2}-m\geq{n'+1\choose2}-{n'\choose2}=n'$ pairs of vertices are non-adjacent, i.e., at least $n'$ edges are missing. 

Suppose $(i,j)\notin E$, and suppose the two vertices have $k$ common neighbors. Notice that $k>0$ as the diameter of $G$ is at most 2. Consider the effect of adding an edge $(i,j)$ into the graph as long as the effect of merging the pair of vertices $(i,j)$.
\begin{description}
\item[Create edge $(i,j)$: ] The number of cycles increases. In particular, we gain $k$ new triangles from the $k$ common neighbors.
\item[Merge vertices $(i,j)$: ] We will gain some cycles and lose some other cycles. In particular, any cycle containing only one or none of $i,j$ remains; any cycle $C$ containing both $i,j$ and whose length is at least 5 changes into one or two shorter cycles $C'$ and $C''$. The changes to these long cycles do good to our objective. Now let's look at some vanishing cycles. Suppose cycle $C$ contains both $i,j$ and has length 4. Then $C$ is of the form $i\ra v\ra j\ra u\ra i$. Merging $(i,j)$ causes $C$ to vanish. Some triangles are also vanishing. Consider two triangles $(i,u,v),(j,u,v)$; after the merge the two triangles become one. These type of the triangles are the only affected ones (proof omitted). After merging $(i,j)$, we also uses $k$ less edges (thanks to the $k$ common neighbors). In summary, among the $k$ common neighbors, if $p$ pairs of them are adjacent, then merging $(i,j)$ causes $p$ triangles vanishing, ${k\choose2}$ cycles of length 4 vanishing, but we can use $k$ more edges to build the graph.
\end{description}

Now back to the graph $G$ and we will show how to merge vertices and add edges. Suppose the non-adjacent pair of vertices are $$(i_1,j_1),\ldots,(i_\alpha,j_\alpha).$$ Recall that $\alpha\geq n'$. Each pair $(i_l,j_l)$ is associated with an integer $k_l$ which is the number of common neighbors. We assume the pairs are sorted in the way that $k_1\geq k_2\geq \cdots\geq k_\alpha$. The procedure is to merge $(i_\alpha,j_\alpha)$ and add some edges to some of the previous non-adjacent pairs.

By previous argument, merging $(i_\alpha,j_\alpha)$ causes $p_\alpha$ triangles and ${k_\alpha\choose2}$ cycles of length 4 vanishing; but we also spares $k_\alpha$ edges that can be added to elsewhere in the graph. Here, $p_\alpha\leq {k_\alpha\choose 2}.$

A natural thought is to add $k_\alpha$ to some of the pairs $(i_1,j_1),\ldots,(i_{\alpha-1},j_{\alpha-1})$ and make some of them adjacent. But notice that a by-product of merging $(i_\alpha,j_\alpha)$ is that it is no longer the case that the pairs $(i_1,j_1),\ldots,(i_{\alpha-1},j_{\alpha-1})$ are non-adjacent. It might be the case that some $i_l=i_\alpha$, and after the merge, the non-edge $(i_l,j_l)=(i_\alpha,j_l)$ changes into $(j_\alpha,j_l),$ and perhaps edge $(j_\alpha,j_l)$ is pre-existing. Hence, we need to upper-bound the decrease in the non-edges $(i_1,j_1),\ldots,(i_{\alpha-1},j_{\alpha-1})$. Suppose after the merge, previous non-edge $(i_l,j_l)$ becomes an edge. Then it must be the case that $i_l=i_\alpha$ and $(j_\alpha,j_l)$ pre-exists (number of such edges is upper-bounded by $|N_{j_\alpha}-N_{i_\alpha}|$), or $j_l=j_\alpha$ and $(i_l,i_\alpha)$ pre-exists (number of such edges is upper-bounded by $|N_{i_\alpha}-N_{j_\alpha}|$). Thus, the number of such edges is upper-bounded by $|N_{j_\alpha}-N_{i_\alpha}|+|N_{i_\alpha}-N_{j_\alpha}|\leq n-2-k_\alpha$. Therefore, previously we have $\alpha-1$ non-adjacent pairs $(i_1,j_1),\ldots,(i_{\alpha-1},j_{\alpha-1})$, after the merge we have at least $\alpha-1-(n-2-k_\alpha)=\alpha-n+1+k_\alpha\geq 1+k_\alpha$ non-adjacent pairs. 

Above argument shows that there are still at least $k_\alpha+1$ pairs remain to be non-adjacent, and the $k_\alpha$ spare edges can be added to some of the non-adjacent pairs. For each such pair $(i_l,j_l),$ adding an edge creates at least $k_l-1\geq k_\alpha-1$ new triangles (minus 1 because $i_\alpha,j_\alpha$ might both appear in the previous common neighbors). Therefore, adding $k_\alpha$ spare edges and make $k_\alpha$ non-adjacent pairs now adjacent creates at least $k_\alpha\cdot (k_\alpha-1)$ new triangles.

In summary, merging $(i_\alpha,j_\alpha)$ kills $p_\alpha$ triangles and $ {k_\alpha\choose 2}$ cycles of length 4, but creates $k_\alpha\cdot (k_\alpha-1)$ new triangles. Since $p_\alpha\leq {k_\alpha\choose 2}$, we get a strictly increasing objective quantity.
\end{proof}

A direct corollary to the above lemma is that, to maximize the expected number of detectable violations in the queries, a tester makes pairwise query on all points they selected. If the number of points in their sample is $o(1\epsilon^{2/3})$, the expected number of violations the tester can find is less than 1. Thus, a lower bound of the query complexity for this hard case instance is $\Omega(1/\epsilon^{4/3})$.





Next, we provide the formal definitions for the three metric spaces of our testing concern.
\begin{definition}[Metric] 
     A distance matrix $M\in\mathbb{R}^{n\times n}$ is a metric if the following conditions hold.

\begin{itemize}
\item \text{Strict metric:} $M(i,j) \ge 0$ $\forall i,j\in[n]$, with $M(i,j)=0$ if and only if $i = j$. 
\item \text{Symmetry:} $M(i,j) = M(j,i)$ $\forall i, j\in[n]$. 
\item \text{Triangle inequality:} $M(i,j)\leq M(i,k) + M(j,k)$ $\forall i,j,k\in[n]$.
\end{itemize}
\end{definition}

\begin{definition}[Ultrametric]
    A distance matrix $M\in \mathbb{R}^{n\times n}$ is an ultrametric if $M$ is a metric and the following condition holds.
    \begin{itemize}
        \item \text{Ultrametric:} $M(i,j)\leq \max\{M(i,k),M(j,k)\}$ $\forall i,j,k\in[n]$.
    \end{itemize}
\end{definition}

\begin{definition}[Tree metric]
    A distance matrix $M\in \mathbb{R}^{n\times n}$ is a tree metric if $M$ is a metric and there exist a graph $G=(V,E)$ and an injection $\phi:[n]\ra V$ such that the following conditions hold.
    \begin{itemize}
        \item $G$ is non-negative, weighted, acyclic, undirected, and connected.
        \item $\forall i\in[n],\phi(i)$ is a vertex in $G$ with degree 1. That is, the image of $\phi$ are the leaves of $G$.
        \item $\forall i,j\in[n],M(i,j)=d(\phi(i),\phi(j)),$ where $d:V\times V\ra \mathbb{R}$ maps a pair of vertices to the length of the unique simple path connecting them in $G$.
    \end{itemize}
\end{definition}

It is not hard to see that an ultrametric is a tree metric, which is a metric.
Ultrametrics and tree metrics are characterised by the 3-point and 4-point conditions respectively. The 3-point condition for ultrametrics is as stated in their definition. The fact that the 4-point condition (defined later) characterises tree metrics is due to Buneman\cite{Buneman}.






\section{Testing General Metrics}\label{sec:general}

In this section we present  an algorithm for testing general metrics with sublinear query complexity $O(n^{2/3}/\epsilon^2)$.
We also give a lower bound construction showing that any testing algorithm, including algorithms with two-sided-error, needs to have query complexity $\Omega(n^{2/3+\nu(n)})$, where $\nu(n)=o(1)$ is a function that goes to 0 at a speed slower than $\log(n)/n$.


\subsection{$O(n^{2/3}/\epsilon^2)$ query complexity upper bound}
We provide a natural testing algorithm with $O(n^{2/3}/\epsilon^2)$ query complexity for testing general metric property of a distance matrix that has success probability higher than $2/3$. The input to the tester is a matrix $M\in(\mathbb{R}^{\geq0})^{n\times n}$, which purportedly is a metric on $[n]$. Recall that in order for $M$ to be a metric it has to satisfy the following conditions.

\begin{itemize}

\item $M(i,j) \ge 0$ $\forall i,j$, with $M(i,j) = 0$ if and only if $i = j$. (Strict metric.)
\item $M(i,j) = M(j,i)$ $\forall i, j$. (Symmetry)
\item $M(i,j) + M(j,k) \ge M(i,k)$ $\forall i,j, k$ (Triangle inequality).

\end{itemize}

Violations to the first two conditions are easy to detect and so we assume that the given matrix is non-negative and symmetric with its diagonal entries being 0. Our tester looks for a witness that the matrix violates triangle inequality. If such a witness is found, the tester outputs ``NON METRIC". Otherwise, it outputs ``METRIC". Thus, since the tester outputs ``NON METRIC'' only when it finds a witness, it always outputs "METRIC" when the input is a metric. Hence, in the following analysis, we assume the given matrix $M$ is $\epsilon$-far from a metric.

The testing algorithm itself is straightforward: Select $s={O}(n^{1/3}/\epsilon)$ points in $[n]$ uniformly at random and query the distance between every pair of selected points. However, the analysis is intricate. We show that, with $s$ vertices in the sample, the expected number of ``bad triangles"  in the sample is a large constant while the variance is small. Then Chebyshev's inequality applies.

The fact that the expected number of violations in our sample is high follows from the claim that each corrupted entry \sk{We haven't defined this yet.} in the distance matrix must be part of a bad triangle. To show the variance is small, on the other hand, requires care. If all bad triangles are concentrated on a small set of vertices or edges, then the success of the tester really depends on whether the sample hits this small set of vertices or edges. Hence, the goal is to rule out this possibility.

Before proceeding to the algorithm and the analysis, we note that instead of a distance matrix, we will be working on an undirected non-negatively weighted graph with $n$ vertices, where the edge weights are defined by the given matrix. That is, for edge $(u,v)$, set weight $w(u,v)=M[u,v]$. In graph terms, $G=(E,V)$ is a metric if it satisfy the following conditions. 
\begin{itemize}
\item $w(e) \ge 0$ $\forall e\in E$. (Strict metric.)
\item $w(a,b)+w(b,c)\geq w(a,c)$ $\forall a,b,c\in V$ (Triangle inequality).
\end{itemize}
Since the given matrix $M$ is $\epsilon$-far from a metric, the corresponding graph $G$ is $\epsilon$-far from a metric in the sense that at least $\epsilon n^2$ edges need to be modified for $G$ to become any metric graph. The tester is looking for evidence to the violation of triangle inequality: three vertices such that the induced 3-cycle violates triangle inequality.

\begin{definition}
    A triangle defined by three vertices $a,b,c$ is bad if $\max(w(a,b),w(a,c),w(b,c))>w(a,b)+w(a,c)+w(b,c)-\max(w(a,b),w(a,c),w(b,c))$.
\end{definition}

Next, we show a relation between the number of bad triangles and the number of edges that need to be fixed for the graph to be a metric. This claim guarantees that the number of bad triangles is not low.
\begin{lemma}
    Let $A$ be the set of bad triangles in the graph $G$. Then $G$ could be fixed into a metric by changing only the weights of edges in $A$.
\end{lemma}
\begin{proof}
    Create another graph $G'$ with the same set of $n$ vertices. For each edge $(u,v)\notin E$, create edge $(u,v)$ in $G'$ with weight same as the edge weight in $G$. If with the current set of edges, $G'$ is disconnected, create an edge between each component of $G'$ with arbitrary weights. Then, for each non-edge $(x,y)$ in $G'$, let its weight be the shortest path distance from $x$ to $y$ in $G'$. Every triangle in $G'$ satisfy triangle inequality, and $G'$ differs from $G$ only at edges in $A$.
\end{proof}

A direct consequence of the above lemma is that, given the fact that at least $\epsilon n^2$ edges of $G$ need to be modified for $G$ to become any metric graph, there are at least $\epsilon n^2/3$ bad triangles in $G$. 

\begin{corollary}\label{corruptionsLeqBadTri}
    If at least $x$ edges of a graph $G$ needs to be fixed for $G$ to be a metric, then there are at least $x/3$ bad triangle in $G$.\qed
\end{corollary}
Let $T$ be a subset of the bad triangles and let $X$ be the number of bad triangles both in $T$ and our sample. Then, if we take $T$ to be some constant fraction of the original set of bad triangles and sample some multiples of $(n/\epsilon)^{1/3}$ vertices, in expectation $X$ is a constant number larger than 1. However, it might not be the case that with high probability $X>1$, as the variance of $X$ might be large.

We could rewrite $X=\sum_{t\in T}I_t$, where $I_t$ is the indicator variable for whether the bad triangle $t\in T$ is included in our sample or not. Then, we could rewrite the variance as
\begin{align*}
    \var[X]=&\e[X^2]-\e[X]^2
    \\=&\e[\sum_{t\in T}I_t+\sum_{t\in T}\sum_{t'\in T,t\neq t'}I_tI_{t'}]-(\sum_{t\in T}\e[I_t])^2
    \\=&\sum_{t\in T}\e[I_t]+\sum_{t\in T}\sum_{t'\in T,t\neq t'}\e[I_tI_{t'}]-\sum_{t\in T}\e[I_t]^2-\sum_{t\in T}\sum_{t'\in T,t\neq t'}\e[I_t]\e[I_{t'}]
    \\=&\sum_{t\in T}P(t\in S)+\sum_{t\in T}\sum_{\substack{t'\in T , t\neq t'}}P(t,t'\in S)-\sum_{t\in T}P(t\in S)^2-\sum_{t\in T}\sum_{\substack{t'\in T , t\neq t'}}P(t\in S)P(t'\in S)
    \\=&\sum_{t\in T}P(t\in S)+\sum_{t\in T}\sum_{\substack{t'\in T , t\neq t', t\cap t'\neq\emptyset}}P(t,t'\in S)-\sum_{t\in T}P(t\in S)^2
    \\\leq &\,\,\e[X]+\sum_{t\in T}\sum_{\substack{t'\in T , \,\,t\neq t'\\ t,t'\text{share a vertex}}}P(t,t'\in S)+\sum_{t\in T}\sum_{\substack{t'\in T ,\,\,t\neq t'\\ t,t'\text{share an edge}}}P(t,t'\in S)
    \\=&\e[X]+\sum_{t\in T}\sum_{\substack{t'\in T , \,\,t\neq t'\\ t,t'\text{share a vertex}}}\left(\frac{(1+o(1))s}{n}\right)^5+\sum_{t\in T}\sum_{\substack{t'\in T ,\,\,t\neq t'\\ t,t'\text{share an edge}}}\left(\frac{(1+o(1))s}{n}\right)^4,
\end{align*}
where the factors $((1+o(1))s/n)^5$ and $((1+o(1))s/n)^4$ come from the fact that when a pair of triangles share a vertex or an edge, their union is 5 or 4 vertices and each vertex has probability $(s/n)$ of being included in the sample. The expectation of $X$ is simply $\e[X]=|T|((1+o(1))s/n)^3$.

To apply Chebyshev's inequality, it suffices to show that $\e[X]$ is a large constant and $\var[X]/\e[X]^2$ is a small constant. Since by the above calculation $\var[X]$ breaks down into three parts, we only need to show that the second term, $(s/n)^5$ times the number of vertex-sharing triangle pairs, and the third term $(s/n)^4$ times the number of edge-sharing triangle pairs, are no larger than some small constants times $\e[X]^2$. That is, the ultimate goal is to find a subset $T$ of bad triangles that satisfy the following conditions.
\begin{equation}
    \e[X]=(s/n)^3\cdot|T|>C,
\end{equation}
\begin{equation}\label{chebyshev:secondterm}
    {(s/n)^{-1}}\cdot|\{(t,t')\in T\times T:t,t'\text{ share a vertex}\}|/|T|^2<c_1,
\end{equation}
\begin{equation}\label{chebyshev:thirdterm}
    (s/n)^{-2}\cdot|\{(t,t')\in T\times T:t,t'\text{ share an edge}\}|/|T|^2<c_2,
\end{equation}
where $C$ is a large constant and $c_1,c_2$ are two small constants.

We first focus on the vertex-sharing pairs. For each vertex, we define its triangle degree $d_T$ to be the number of bad triangles in $T$ this vertex participates in. That is,
\begin{definition}
    Given a subset $T$ of bad triangles, the triangle degree of a vertex $v$ is defined to be $d_T(v):=|\{t\in T,v\in t\}|$. If not specified, $T$ is the set of all bad triangles in the current graph.
\end{definition}
Then, it is not hard to see that $\sum_{v\in V}d_T(v)=3|T|$. Moreover, the number of vertex-sharing triangle pairs in $T$ is $\sum_{v\in V}{d_T(v)\choose2}\leq\sum_{v\in V} d_T(v)^2/2$. Hence, to show relation~\ref{chebyshev:secondterm} holds, it suffices to make $$(s/n)^{-1}\cdot \frac{\sum_{v\in V}d_T(v)^2}{(\sum_{v\in V}d_T(v))^2}$$ a small constant. Notice, however, that if no constraint is set on $d_T(v)$, it could get as large as $\Omega(n^2)$ and, as a consequence, the above quantity is large. Hence, the first phase of the testing algorithm is a ``pre-screening" phase which rules out the scenario that many vertices have high triangle degree.

\begin{algorithm}
\caption{Metric Testing (part one)}\label{algo:metric1}
\begin{algorithmic}

\Statex
\Procedure{HighDegreeDetection}{$G=(U,V)$}
\State\Comment{$G$ is an undirected, non-negatively weighted clique on $n$ vertices}
\State $V'\gets 3/\epsilon^{1.1}$ vertices sampled uniformly at random
\State $E'\gets 12n^{2/3}$ edges sampled uniformly at random
\For {each pair $(v,e)\in V'\times E'$}
\State Test triangle inequality on the triangle formed by the vertex $v$ and edge $e$
\If {violtate triangle inequality}
\State\Return NON-METRIC
\EndIf
\EndFor
\State\Return SUCCEEDED
\EndProcedure
\end{algorithmic}
\end{algorithm}

\begin{claim}
    If the input graph $G$ has more than $\epsilon^{1.1} n$ vertices with at least $n^{4/3}/4$ triangle degree, Algorithm~\ref{algo:metric1} returns SUCCEEDED with probability at least 5/6.
\end{claim}
\begin{proof}
    In the proof, we denote vertices with triangle degree at least $n^{4/3}/4$ ``high-degree vertices". The probability that no high degree vertex is sampled in $V'$ is at most $(1-\epsilon^{1.1})^{3/\epsilon^{1.1}}\leq e^{-3}$. With probability larger than $1-e^{-3}$, a high degree vertex falls into $V'$, and it forms bad triangles in $T$ with at least $n^{4/3}/4$ edges. Thus, a random sample $E'$ hits at least one of these edges with probability at least $1-(1-n^{-2/3}/4)^{12n^{2/3}}\geq 1-e^{-3}$. By union bound, with probability at least 5/6 Algorithm~\ref{algo:metric1} detects such a (vertex, edge) pair that forms a bad triangle in $T$ and returns SUCCEEDED.
\end{proof}

From now on, suppose that the number of high degree vertices (vertex whose triangle degree is at least $n^{4/3}/4$) is smaller than $\epsilon^{1.1}n$. Below, we propose a easy fix to $G$ which implies that there exists a great amount of bad triangles such that when defining triangle degree over this set, the triangle degree of any vertex is low. With this guarantee, we only use these bad triangles as testing evidence to control the variance of $X$ that is contributed by vertex-sharing pairs of triangles.

\begin{lemma}\label{lowVertexDegree}
    Suppose in $G$, the number of vertices whose triangle degree (defined over the entire set of bad triangles) is at least $n^{4/3}/4$ is smaller than $\epsilon^{1.1}n$, then there is a set $\overline{T}$ of at least $\epsilon n^2/15$ bad triangles such that for any vertex $v\in V$, $d_{\overline{T}}(v)< n^{4/3}/4$. The notation $\overline{T}$ is used later in the analysis.
\end{lemma}
\begin{proof}
    Let $U$ be the set of high degree vertices in $G$. Consider the graph $\overline{G}=(V,\overline{E})$ which is on the same set of vertices as $G$. For edge $(a,b)$ where both endpoints $a,b$ are not in $U$, define the weight of $(a,b)$ in $\overline{G}$ to be the same as the weight in $G$. For all other edges, define their weight in $\overline{G}$ to be $\infty$. Then, $\overline{G}$ differs from $G$ at at most $|U|n\leq \epsilon^{1.1}n^2$ edges. Since $G$ is $\epsilon$-far from a metric, $\overline{G}$ must be $(\epsilon-\epsilon^{1.1})$-far from a metric. Otherwise, there is a fix on no more than $(\epsilon-\epsilon^{1.1})n^2$ edges of $\overline{G}$ that makes it a metric; as a result, there is a fix on no more than $\epsilon n^2$ edges of $G$ that makes it a metric.

    By \hyperref[corruptionsLeqBadTri]{Corollary~\ref{corruptionsLeqBadTri}}, since $\overline{G}$ is $(\epsilon-\epsilon^{1.1})$-far from a metric, there are at least $(\epsilon-\epsilon^{1.1})n^2/3\geq \epsilon n^2/15$ bad triangles in $\overline{G}$, for $\epsilon<0.1$. But any triangle touching at least one vertex in $U$ is not bad: edges incident to vertices in $U$ is set to $\infty$, so these triangles obey triangle inequality. Therefore, all $\epsilon n^2/15$ bad triangles use solely the vertices in $V\backslash U$. By design, these triangles have their one-to-one copies in $G$. Let $\overline{T}$ be this set of bad triangles. Notice that every vertex in $G$ is included in less than $n^{4/3}/4$ bad triangles in $\overline{T}$: each vertex $u\in U$ is included in none; each vertex $v\in V\backslash U$ is included in less than $n^{4/3}/4$ bad triangles in $G$, and so less than $n^{4/3}/4$ bad triangles in $\overline{T}$. Thus, $d_{\overline{T}}(v)<n^{4/3}/4$ for all $v\in V$. The claim follows.
\end{proof}

Following this result, we find a great number of bad triangles ``spread almost evenly" among the low degree vertices. Hence, to simplify the analysis, we assume the high triangle degree vertices in $U$ is removed from $G$, and we only care about the induced subgraph of $G\backslash U$.  The variance of $X$ due to vertex-sharing pairs can be upper bounded as long as the set of bad triangles $T$ we use is a constant subset of $\overline{T}$. This is because, with an upper bound on each $d_T(v)$, by convexity the below quantity can be upper bounded by a constant.
\begin{equation*}
    {(s/n)^{-1}}\cdot|\{(t,t')\in T\times T:t,t'\text{ share a vertex}\}|/|T|^2\sim  (s/n)^{-1}\cdot \frac{\sum_{v\in V}d_T(v)^2}{(\sum_{v\in V}d_T(v))^2}
\end{equation*}


At this point, we find a large set of bad triangles such that the variance of $X$ induced by vertex-sharing triangles in this set is controlled. In the later half of this section, we show that we can further prune this set of triangles such that the variance induced by edge-sharing triangles is upper bounded.

Recall that the third relation we hope to achieve is 
\begin{equation*}
    (s/n)^{-2}\cdot|\{(t,t')\in T\times T:t,t'\text{ share an edge}\}|/|T|^2<c_2.
\end{equation*}
Previously, triangle degree is a function on vertices. We now extend domain to include all the edges. In this way, the number of edge-sharing triangle pairs can be expressed as a formula of triangle degree of edges.
\begin{definition}
    Given a subset $T$ of bad triangles, the triangle degree of an edge $e$ is defined to be the number of bad triangles in $T$ the edge participates in. That is, $d_T(e):=|\{t\in T,e\in t\}|$. If not specified, $T$ is the set of all bad triangles in the current graph.
\end{definition}
Then, the number of edge-sharing triangle pairs in a set $T$ is simply $\sum_{e\in E}{d_T(e)\choose 2}\leq \sum_{e\in E}d_T(e)^2/2$. The number of bad triangle s in $T$ is $|T|=\sum_{e\in E}d_T(e)/3$. Analogously, the third relation is achieved if the quantity $$(s/n)^{-2}\cdot \frac{\sum_{e\in E}d_T(e)^2}{(\sum_{e\in E}d_T(e))^2}$$ is a small constant.

One useful relation between triangle degree of edges and triangle degree of vertices is that, $$d_T(v)=\sum_{e:\,e\text{ incident to }v}d_T(e)/2.$$ From previous results, the triangle degree of each vertex is bounded by $d_{\overline{T}}(v)< n^{4/3}/4$. This indicates that the $\Omega(n)$ edges incident to $v$ cannot all have high triangle degree. But this is not enough, as there can still be non-negligible amount of incident edges having triangle degree close to $n$. In this case we do not have a good bound on the variance.

However, when an edge happens to have a high triangle degree, intuitively we can modify this edge to fix many triangles. This intuition is the core of the later arguments. We show below that there exist ways to fix high triangle degree edges to make their degree lower. Then, with a few amount of fixes, the modified graph still have a good amount of bad triangles that allow us to bound the variance.

First, let us define quantitatively what is a high triangle degree edge.
\begin{definition}
    Given a subset $T$ of bad triangles, if $d_T(e)>4n^{2/3}$, the edge $e$ is a high triangle degree edge. As a simplification, we refer to it as a heavy edge. With respect to the set $\overline{T}$ of bad triangles defined in Lemma~\ref{lowVertexDegree}, let $\overline{E}$ be the set of all heavy edges in $G$.
\end{definition}
Recall that, $\overline{T}$ is the set of all bad triangles in the graph $G\backslash U$; in the following analysis, we ignore all vertices in $U$. Since each vertex has triangle degree less than $n^{4/3}/4$, there can be at most $n^{2/3}/8$ incident heavy edges, deriving from the relation between $d_T(e)$ and $d_T(v)$ above. Thus, we have an upper bound on the set of all heavy edges $|\overline{E}|<n^{5/3}/16$.

We claim that, for any heavy edge $e\in \overline{E},$ there is a value we can set the weight of $e$ to be such that now $e$ is incident to at most $n^{2/3}$ bad triangles. That is, in the new graph with only one weight change, the triangle degree of $e$ is significantly lower.

\begin{lemma}\label{changeEdgeFixTriangle}
    For any heavy edge $e=(x,y)\in \overline{E}$, there exists a weight value such that if $w(e)$ is modified to be this new weight, at most $n^{2/3}$ triangles incident to $e$ are bad triangles.
\end{lemma}
\begin{proof}
    The edge $e$ is incident to $n-2$ triangles, each can be represented as $(x,y,v_i)$ for some $i\in[n-2]$. The statement follows from the below lemma.
    \begin{claim}\label{lem:intervals}
        Suppose the edge $e$ is incident to a set of triangles. If for any weight value in $[0,\infty]$ edge $e$ takes on, at least $t$ of the incident triangles remain to be bad, then there are at least $t^2/2$ pairs of vertices $(v_i,v_j)$ for $i,j\in[n-2]$ such that at least one of the triangles $(v_i,v_j,x),(v_i,v_j,y)$ is bad.
    \end{claim}
    Suppose the lemma holds. We take $t$ to be $n^{2/3}$. If no matter what weight we set $e$ to be, at least $t=n^{2/3}$ incident triangles are bad, then there exist at least $n^{4/3}/2$ edges, each of them forms a bad triangle with either $x$ or $y$. By pigeon hole theorem, we have a contradiction since the triangle degrees of both $x$ and $y$ are smaller than $n^{4/3}/4$. Thus, we are done if the lemma holds.
    \begin{proof}[Proof of claim]
        For each triangle $(x,y,v_i)$ the edge $e=(x,y)$ incident to, $v_i$ ``sets an interval" to the possible weights $e$ can take on for the triangle to be good. This interval is exactly $[|w(x,v_i)-w(y,v_i)|,w(x,v_i)+w(y,v_i)]$. The triangle is good if and only if the weight of $e$ lands within the interval. Thus, the problem of finding a weight for $e$ to make as many as the incident triangles good boils down to find a value that hits as many as these $n-2$ intervals as possible. For any weight $w$ the edge $e$ takes on, there are at least $t$ bad incident triangles; this is equivalent to saying the value $w$ lies outside at least $t$ intervals, or lies within less than $(n-2)-t$ intervals. We will then show that if there is no value that hits at least $(n-2)-t$ intervals, then there must be at least $t^2/2$ pairs of pair-wise disjoint intervals.

        Imagine that we sort all the intervals by the starting point, and imagine a value $p$ going from 0 to $\infty$. At any point in time, $p$ lies within less than $(n-2)-t$ intervals. For the first time $p$ leaves some interval $I_1$, there are still at least $t$ intervals $p$ hasn't encountered yet, which implies $I_1$ is disjoint from these $t$ intervals, giving us $t$ pairs of disjoint intervals. In general, when $p$ leaves the $j^{th}$ interval, there are at least $t-j+1$ intervals that $p$ hasn't intersect, meaning the $j^{th}$ interval is disjoint from these $t-j+1$ intervals. Therefore, there exist at least $t^2/2$ pairs of pair-wise disjoint intervals.

        Now, suppose the two intervals imposed by two vertices $v_i,v_j$ are disjoint. Without loss of generality, we assume that $|w(x,v_i)-w(y,v_i)|\leq w(x,v_i)+w(y,v_i)<|w(x,v_j)-w(y,v_j)|\leq w(x,v_j)+w(y,v_j)$. Then, from the middle inequality, it must be the case that either $w(x,v_j)>w(x,v_i)+w(y,v_i)+w(y,v_j)$ or $w(y,v_j)>w(x,v_i)+w(y,v_i)+w(x,v_j)$. Intuitively, it means the 4-cycle $(x,v_i,y,v_j)$ is ``bad". Suppose we are in the case that $w(x,v_j)$ is heavier than the sum of other three edges. (The other case that $w(y,v_j)$ is the heaviest follows the same analysis.) Then, it must be the case that either $w(x,v_j)>w(x,v_i)+w(v_i,v_j)$ or $w(v_i,v_j)>w(y,v_i)+w(y,v_j)$. In former case edge $(v_i,v_j)$ forms a bad triangle with $x$ while in the latter case edge $(v_i,v_j)$ forms a bad triangle with $y$.

        Combining all the above arguments, there are at least $t^2/2$ pairs of pairwise disjoint intervals. Each pair corresponds to a unique pair of vertices $(v_i,v_j)$ for $i,j\in[n-2].$ Each such pair of vertex corresponds to an edge that forms a bad triangle with either $x$ or $y$. The lemma follows.
    \end{proof}
\end{proof}

With this useful lemma in hand, we propose a fixing procedure, where we only touch the heavy edges in $\overline{E}$ to fix as many as incident triangles as possible. Recall that $|\overline{E}|\leq n^{5/3}/16$, so this fixing procedure only cost us a little.

First, we set an arbitrary order on the heavy edges in $\overline{E}=\{e_1,...,e_k\}$. Then, following this order, we change each $e_i\in \overline{E}$ in the fashion that the triangles incident to $e_i$ are fixed as many as possible. After changing all $|\overline{E}|$ edges, we obtained a new graph $G'$. Since only $|\overline{E}|\leq n^{5/3}/16$ changes have been made on $G$, at least $\epsilon n^2-n^{5/3}/16$ edges need to be modified on $G'$ for it to be a metric. By Corollary~\ref{corruptionsLeqBadTri}, there are at least $\epsilon n^2/6$ bad triangles in $G'$. 
\begin{algorithm}
\label{algo:fix}
\begin{algorithmic}
\Statex
\Procedure{FixingProcedure}{$G=(U,V)$}
\State\Comment{$G$ is an undirected, non-negatively weighted clique on $n$ vertices}
\State\Comment{Assume $G$ has no vertex with triangle degree higher than $n^{4/3}/4$}
\State $\overline{E}\gets$ initialize an empty set
\State $\mathcal{T}\gets$ all bad triangles in $G$
\State $G'\gets$ copy of $G$
\For {$e\in E$}
\If{$e$ is in at least $4n^{2/3}$ triangles in $\mathcal{T}$}
\State Add $e$ to $\overline{E}$
\EndIf
\EndFor
\For {each $e\in\overline{E}$}
\If {$e$ is in at least $4n^{3/2}$ bad triangles in current $G'$}
\State Change the weight of $e$ such that the number of good incident triangles is as high as possible
\State Update the weight of $e$ in $G'$
\EndIf
\EndFor
\State\Return $G'$
\EndProcedure
\end{algorithmic}
\end{algorithm}

It seems like we are now in a good shape: we have a good amount of bad triangles and the triangle degree for each edge is controlled below $4n^{2/3}$. The variance argument should work out. However, there are some subtleties that need to be addressed.
\begin{enumerate}
    \item After changing edges $e_1,...,e_l$, does the result in Lemma~\ref{changeEdgeFixTriangle} still hold? Namely, changing an edge $e_i$ indeed would lower the total amount of bad triangles, but it is possible that this procedure sacrifices some good incident triangles to fix more bad incident triangles. With the changed weights, is it still the case that the weight of $e$ can be set to some value so that no more than $n^{2/3}$ incident triangles are good?
    \item Since the procedure might make some good triangles bad, the bad triangles in $G'$ might be mostly good in $G$. In that case, these triangles are useless for our analysis.
    \item Suppose we have the guarantee that we could change $e_i$ so that no more than $n^{2/3}$ incident triangles are bad. But as we change $e_{i+1},e_{i+2}$ and so on, we might introduce some bad triangles who are incident to $e_i$. Over the time, the triangle degree of $e_i$ in $G'$ is still unbounded.
\end{enumerate}
Fortunately, the above scenarios will never happen, and we provide below a sequence of detailed analysis, leading to a success in finding the desired set of bad triangles. We will start with addressing the first issue. The below lemma is a stronger version of Lemma~\ref{changeEdgeFixTriangle}, which states that after changing the weights for the first $l-1$ edges in $\overline{E}$, it remains to be true that the $l^{th}$ edge can be fixed so that it is now incident to no more than $n^{2/3}$ bad triangles.

\begin{lemma}\label{strongChangeEdgeFixTriangle}
    After changing the edges $e_1,...,e_{l-1}$, each aiming to make the number of incident bad triangles as small as possible, there exists a weight value for $e_l$ such that with this weight, there are at most $n^{2/3}$ bad triangles incident to $e_l$.
\end{lemma}
\begin{proof}
    We will have the claim if we can show that after changing the edges $e_1,...,e_j$ in the proposed way for all $j\in[l-1],$ $w(e_l)$ could be set to some value so that at most $n^{2/3}$ incident triangles are bad. We prove by induction.

    The base case is clear: if no edges have been changed yet, the statement is exactly Lemma~\ref{changeEdgeFixTriangle}.

    Suppose after changing $e_1,...,e_j$, we can still find a value for $w(e_l)$ such that the number of incident bad triangles is bounded. Now the fixing procedure moves on to $e_{j+1}$. Suppose that the endpoints of edge $e_l=(x,y)$. Then, if $e_{j+1}$ is not incident to either $x$ or $y$, changing $e_{j+1}$ has no influence on $e_l$ and its incident triangles, so the statement follows from the inductive hypothesis. Thus, without loss of generality, we suppose $e_{j+1}=(x,v_i)$. In the proof of Lemma~\ref{changeEdgeFixTriangle}, we have shown that if the weight of edge $e_l$ cannot be tuned to some value so that at most $n^{2/3}$ incident triangles are bad, then at least $n^{4/3}/2$ edges of the form $(v_s,v_r)$ where $v_s,v_r\in V\backslash\{x,y\}$ constitute bad triangles with either $x$ or $y$. On the other hand, after modifying $e_{j+1}=(x,v_i)$, the triangles formed by vertex $y$ and the edges $(v_s,v_r)$ remain uninfluenced. If neither $v_s,v_r$ is $v_i$, then the triangle formed by the edge $(v_s,v_r)$ and vertex $x$ remains uninfluenced. Since $e_{j+1}=(x,v_i)$ is modified in a way that the number of incident bad triangles strictly decreases, the number of edges $(v_i,v_r)$ that form a bad triangle with vertex $x$ is non-increasing. Thus, we still have the situation that the number of edges $(v_s,v_r)$ forming a bad triangle with either $x$ or $y$ is less than $n^{4/3}/2$. Thus, modifying $e_{j+1}$ will not harm $e_l$: there is still a way to modify $e_l$ such that at most $n^{2/3}$ triangles incident to $e_l$ are bad.
\end{proof}

After the above result, we have the guarantee that, through out the fixing procedure, as soon as an edge $e_l$ is modified, at most $n^{2/3}$ triangles incident to $e_l$ is bad. Now, we provide below a guarantee that with $\epsilon n^2/6$ bad triangles in $G'$, we could recover a great amount of bad triangles in $G$ such that the number of edge-sharing pairs is upper bounded.
\begin{lemma}\label{readjustTriangles}
    After changing all the heavy edges in $\overline{E}$ in the way proposed in the fixing procedure, graph $G'$ is obtained. Given a set $T'$ of bad triangles in $G'$, there exists a set $T$ of bad triangles in $G$ such that $|T|=|T'|$ and $d_T(e)\leq 4n^{2/3}$ for all $e\in G$.
\end{lemma}
\begin{proof}
    Suppose the set of heavy edges is $\overline{E}=\{e_1,...,e_k\}$, and the fixing procedure proceeded with this order. We propose below a ``re-adjusting procedure" which go through the edges in the order $\{e_k,...,e_1\}$, replace the triangles $t'\in T'$ incident to edge $e_i$ with another set of triangles $t\in T$ also incident to $e_i$ and are bad in $G$.

    This re-adjusting procedure satisfies the following conditions:
    \begin{enumerate}
        \item The re-adjusting procedure go through the set of heavy edges in the order $e_k,e_{k-1},...,e_1$.
        \item Let $T^i$ be the set of triangles (each one could be good or bad) after re-adjusting for $e_k,...,e_{i+1}$ and before re-adjusting for $e_{i}$. The beginning set $T^k$ is initialized to $T'$, the set of all bad triangles in $G'$. After re-adjusting for all edges in $\overline{E}$, triangle set $T$ is obtained.
        \item As the re-adjusting procedure reaches edge $e_i$, no more than $n^{2/3}$ triangles in $T^i$ are incident to $e_i$. Let $A_i$ be this set of incident triangles.
        \item There exists a set of triangles $B_i$ such that $B_i$ and each triangle $t\in B_i$ satisfies below conditions:
        \begin{itemize}
            \item $t$ is bad in $G$; 
            \item $t$ is incident to $e_i$; \item two other edges of $t$ are non-heavy edges in $E\backslash \overline{E}$;
            \item $B_i\cap T^i=\emptyset$; and so $B_i\cap A_i = \emptyset$;
            \item $|A_i|=|B_i|$.
        \end{itemize} 
        The re-adjusting procedure defines the new set of triangles $T^{i-1}$ to be $(T^i\backslash A_i)\cup B_i$; finishes the re-adjustment for $e_i$; and moves on to re-adjust for $e_{i-1}$.
    \end{enumerate}
    We show by induction on the set of triangles $T^i$ obtained in each iteration that such re-adjusting procedure exists and is valid.

    For the base case, the procedure initialize the set of triangles $T^k$ to be $T'$, the set of all bad triangles in $G'$. Since $e_k$ is the last edge considered in the fixing-procedure, after changing the edge weight of $e_k$ we obtained the final graph $G'$. Recall that in the fixing procedure, $e_k$ is changed to a value such that as little as the incident triangles are bad. By Lemma~\ref{strongChangeEdgeFixTriangle}, there exists a weight value for $e_k$ such that at most $n^{2/3}$ triangles incident to $e_k$ are bad. Thus, in $G'$, there are at most $n^{2/3}$ bad triangles incident to $e_k$. Since $T^k$ is the set of all bad triangles in $G'$, as a consequence, at most $n^{2/3}$ triangles in $T^k$ are incident to $e_k$, and the third bullet point follows. Let $A_k$ denote this small set of incident triangles. By definition of heavy edges, $e_k$ is incident to at least $4n^{2/3}$ bad triangles in $G$. Recall that the low-triangle-degree for each vertex implies that each vertex is incident to at most $n^{2/3}/8$ heavy edges; in particular it is the case for each of the two endpoints of $e_k$. By pigeon hole theorem, among the $4n^{2/3}$ bad triangles in $G$ incident to $e_k$, at least $15/4n^{2/3}$ of them have some non-heavy second and third edges. Moreover, at least $11/4n^{2/3}$ of them are not in $A_k$ because $A_k$ has size at most $n^{2/3}$. Given these facts, there exists a subset $B_k$ of these $11/4n^{2/3}$ triangles where $|B_k|=|A_k|\leq n^{2/3}$. The fourth bullet point then follows, and we define $T^{k-1}=(T^k\backslash A_k)\cup B_k$.

    For inductive steps, assume we have followed the re-adjusting procedure to re-adjust for edges $e_k,...,e_{i+1}$, and the four conditions hold throughout this process. Now we obtain a set of triangles $T^i$ and start re-adjust for edge $e_i$. We want to show the third bullet point holds, that there are no more than $n^{2/3}$ triangles in $T^i$ incident to $e_i$. Notice that any triangle $t\in T^i$ incident to $e_i$ does not have any of the edges $e_{i+1},e_{i+2},...,e_k$. This is by the inductive hypothesis: any triangle incident to $e_{i+1}$ in $T^i$, for example, only uses edge $e_{i+1}$ and edges in $E\backslash \overline{E}$. Because $e_i\in \overline{E}$ is a heavy edge, any triangle in $T^i$ cannot use $e_i,e_j$ at the same time for all $j>i$. Therefore, triangles in $T^i$ incident to $e_i$ can only be the bad triangles in $G'$ that do not contain $e_j$ for any $j>i$. Recall that immediately after fixing $e_i$ in the fixing procedure, there are at most $n^{2/3}$ bad triangles incident to $e_i$. Some of them might become good when fixing latter heavy edges $e_{i+1},...,e_k$, and some good incident triangles might become bad in $G'$. For any good incident triangles that becomes bad in future fixes, it must contain some $e_j$ for $j>i$, otherwise changing $e_{i+1},...,e_k$ will have no influence on it. However, this triangle is not included in $T^i$ by the above argument (as they contain both $e_i$ and $e_j$). Therefore, the triangles incident to $e_i$ in $T^i$ is a subset of the bad incident triangles obtained immediately after fixing $e_i$, which has size at most $n^{2/3}$. The third bullet point follows. The proof for the fourth bullet point is similar to that in the base case analysis. Since $e_i$ is incident to at least $4n^{2/3}$ bad triangle in $G$ thanks to its heavy edge identity, at least $15/4n^{2/3}$ of them use only edge $e_i$ and non-heavy edges in $E\backslash\overline{E}$. At least $11/4n^{2/3}$ of them are not in $A_i$, the current set of triangles incident to $e_i$. Thus, we can find a set $B_i$ of size $|A_i|\leq n^{2/3}$ among these $11/4n^{2/3}$ triangles that satisfy the properties in the fourth bullet point. Then, define the new set of triangles $T^{i-1}$ to be $(T^i\backslash A_i)\cup B_i$. We are then done with re-adjusting for $e_i$ and the fourth bullet point follows.

    By the above induction, the re-adjusting procedure satisfy the proposed conditions. In the end, we obtain a set $T$ of bad triangles, and we are left to show that $T$ satisfy the properties in the lemma statement. That is, 
    \begin{itemize}
        \item Every triangle $t\in T$ is a bad triangle in $G$;
        \item $|T|=|T'|$;
        \item $d_T(e)\leq 4n^{2/3}$ for all $e\in G$.
    \end{itemize}
    
    First, if the triangle $t\in T$ contains some heavy edge $e_i$, then its membership in $T$ must due to $T^i$, the time we re-adjust for $e_i$. It implies that $t\in B_i$, a subset of bad triangles in $G$. If, on the other hand, $t\in T$ does not contain any heavy edge. Then through out the fixing process, $t$ is untouched so its good-or-bad identity is not changed. Moreover, this triangle is untouched throughout the re-adjusting procedure as the procedure only cares about triangles who use at least one heavy edge. Thus, its membership in $T$ implies its membership in $T^k=T'$, further implies that $t$ is bad in $G'$, finally implies that $t$ is bad in $G$. Thus, $T$ is indeed a subset of bad triangles in $G$.

    Second, notice that throughout the re-adjusting procedure, the size of $T^i$ remains the same. This is because every time we re-adjust for an edge, some set of triangles is removed, and another set of triangles with same cardinality is added. Therefore, $|T|=|T^1|=\cdots=|T^k|=|T'|$.

    Third, we do a case analysis on whether $e$ is non-heavy or heavy. If $e$ is non-heavy, it is incident to at most $4n^{2/3}$ bad triangles in $G$, so as $T$ is a subset of bad triangles in $G$, $d_T(e)\leq 4n^{2/3}$. Now suppose $e$ is heavy. It is included in the re-adjusting procedure as some $e_i$. When re-adjusting for $e_i$, at most $n^{2/3}$ triangles incident to $e_i$ are present in $T^{i-1}$. Moreover, later in the re-adjusting procedure, no triangles incident to $e_i$ is added. Thus, there are at most $n^{2/3}$ triangles incident to $e=e_i$ in $T$.

    The claim follows.
\end{proof}

As a summary, the re-adjusting procedure proposed in Lemma~\ref{readjustTriangles} is as below.
\begin{algorithm}
\label{algo:readjust}
\begin{algorithmic}
\Statex
\Procedure{ReAdjustingProcedure}{$G=(U,V),G'=(U',V'),\overline{E}$}
\State\Comment{$G$ is an undirected, non-negatively weighted clique on $n$ vertices}
\State\Comment{Assume $G$ has no vertex with triangle degree higher than $n^{4/3}/4$}
\State\Comment{$G'$ is the output of $FixingProcedure(G)$}
\State\Comment{$\overline{E}$ is a set of all heavy edges in $G$ sorted in the order used in the Fixing Procedure}
\State $T'\gets$ all bad triangles in $G'$
\State $\mathcal{T}\gets$ all bad triangles in $G$
\For {$e\in $ reverse order of $\overline{E}$}
\State $A\gets$ triangles in $T'$ which are incident to $e$
\State $B'\gets$ triangles in $\mathcal{T}$ which are incident to $e$ and use only edges in $\{e\}\cup(E\backslash\overline{E})$
\State $B\gets$ a subset of $B'$ of the same size as $A$
\State $T'\gets (T'\backslash A)\cup B$
\EndFor
\State $T\gets T'$
\State\Return $T$
\EndProcedure
\end{algorithmic}
\end{algorithm}

The Fixing Procedure along with the above lemma guarantee the existence of an ideal set of bad triangles in $G$, such that each vertex and edge participates in a small amount of triangles. 

\begin{lemma}
    Suppose for a graph $G$, there are less than $\epsilon^{1.1}n$ vertices who participate in more than $n^{4/3}/4$ bad triangles. There exists a set $T$ of $\epsilon n^2/30$ bad triangles in $G$ such that for each vertex $v\in V$, $d_T(v)\leq n^{4/3}/4$; for each edge $e\in E$, $d_T(e)\leq 4n^{2/3}$.
\end{lemma}
\begin{proof}
    As shown in Lemma~\ref{lowVertexDegree}, we could remove the $\epsilon^{1.1}n$ vertices and obtain a graph $\overline{G},$ where there are at least $\epsilon n^2/15$ bad triangles in $\overline{G}$ and each vertex participates in no more than $n^{4/3}/4$ of them. More specifically, at least $\epsilon n^2-\epsilon^{1.1}n^2$ edges in $\overline{G}$ need to be fixed for $\overline{G}$ to become a metric. After the Fixing Procedure we obtain $G'$ from $\overline{G}$ with less than $n^{5/3}/16$ modifications. Thus, in total less than $\epsilon n^2/10$ changes have been made, so by Corollary~\ref{corruptionsLeqBadTri}, $G'$ has at least $\epsilon n^2/30$ bad triangles. Following Lemma~\ref{readjustTriangles}, there exists a set $T$ of $\epsilon n^2/30$ bad triangles in $\overline{G}$ such that $d_T(e)\leq 4n^{2/3}$. Hence, in graph $G$, each vertex participates in at most $n^{4/3}/4$ bad triangles in $T$ and each edge participates in at most $4n^{2/3}$ bad triangles in $T$.
\end{proof}

With this set of bad triangles spreading evenly in the graph $G$, we could proceed with the variance argument and prove that $O(n^{1/3}/\epsilon^2)$ vertices sample is sufficient to hit a bad triangle with high probability.

\begin{lemma}
    Suppose the graph $G$ has less than $\epsilon^{1.1}n$ vertices who participate in more than $n^{4/3}/4$ bad triangles. Then with $s=O(n^{1/3}/\epsilon)$ vertices samples, at least one bad triangle appears in the sample with high probability.
\end{lemma}
\begin{proof}
    Using the previous lemma, we find a set $T$ of $\epsilon n^2/30$ bad triangles in $G$ such that for each vertex $v\in V$, $d_T(v)\leq n^{4/3}/4$; for each edge $e\in E$, $d_T(e)\leq 4n^{2/3}$. As before, let $X$ be the random variable that counts the number of bad triangles in the sample set $S$. In expectation, the number of detected bad triangles $\e[X]=(s/n)^3\cdot\epsilon n^2/30$ is a large constant when $s$ is at least a large constant multiples of $(n/\epsilon)^{1/3}$.

    As argued before, we are done if we can show that $\var[X]/\e[X]^2$ is a small constant, and it boils down to showing the two inequalities~\ref{chebyshev:secondterm} and~\ref{chebyshev:thirdterm}:
\begin{equation*}
    {(s/n)^{-1}}\cdot|\{(t,t')\in T\times T:t,t'\text{ share a vertex}\}|/|T|^2<c_1,
\end{equation*}
\begin{equation*}
    (s/n)^{-2}\cdot|\{(t,t')\in T\times T:t,t'\text{ share an edge}\}|/|T|^2<c_2.
\end{equation*}
Now we rewrite the terms in these relations using triangle degrees, which are bounded in our set of triangles $T$. That is, we have the following relations. $$|T|=\sum_{v\in V}d_T(v)/3=\sum_{e\in E}d_T(e)/3=\epsilon n^2/30$$
$$|\{(t,t')\in T\times T:t,t'\text{ share a vertex}\}|=\sum_{v\in V}{d_T(v)\choose 2}\leq \sum_{v\in V}d_T(v)^2/2$$
$$|\{(t,t')\in T\times T:t,t'\text{ share an edge}\}|=\sum_{e\in E}{d_T(e)\choose 2}\leq \sum_{e\in E}d_T(e)^2/2$$
Now, the left hand sides of the two inequalities, respectively, are no larger than 
$$(s/n)^{-1}\cdot\frac{\sum_{v\in V}d_T(v)^2/2}{(\sum_{v\in V}d_T(v)/3)^2}\leq (s/n)^{-1}\cdot c\frac{\epsilon n^{2/3}\cdot(n^{4/3})^2}{(\epsilon n^{2/3}\cdot n^{4/3})^2}=c\frac{n^{1/3}}{s\cdot\epsilon},$$
$$(s/n)^{-2}\cdot\frac{\sum_{e\in E}d_T(e)^2/2}{(\sum_{e\in E}d_T(e)/3)^2}\leq (s/n)^{-2}\cdot c'\frac{\epsilon n^{4/3}\cdot (n^{2/3})^2}{(\epsilon n^{4/3}\cdot n^{2/3})^2}=c'\frac{n^{2/3}}{s^2\cdot\epsilon}.$$
Thus, both are less than a small constant if we take $s$ to be a large constant multiples of $n^{1/3}/\epsilon$. Since $\var[X]/\e[X]$ is small and $\e[X]$ is large, Chebyshev's inequality applies and $P(X>0)>5/6$.
\end{proof}

Now, we provide the second part of the testing algorithm. Together with the first part, the algorithm successfully detects a bad triangle with probability least 2/3 by union bound.
\begin{algorithm}
\caption{Metric Testing (part two)}\label{algo:metric2}
\begin{algorithmic}
\Procedure{BadTriangleDetection}{$G=(U,V)$}
\State\Comment{$G$ is an undirected, non-negatively weighted clique on $n$ vertices}
\If{procedure HighDegreeDetection($G$) returns NON-METRIC}
\State\Return NON-METRIC
\EndIf
\State $S\gets C\cdot n^{1/3}/\epsilon$ vertices sampled uniformly at random, $C$ is a large constant
\State $E_S\gets$ query pair-wise distance of points in $S$
\For {each 3-tuple $(a,b,c)\in S$}
\State test triangle inequality on the triangle formed by $(a,b,c)$ using knowlegde in $E_S$
\If {violtate triangle inequality}
\State\Return NON-METRIC
\EndIf
\EndFor
\State\Return METRIC
\EndProcedure
\end{algorithmic}
\end{algorithm}

\begin{thm}
    The algorithm Metric Testing takes in an input graph $G$, makes $O(n^{1/3}/\epsilon^2)$ queries on edges in $G$, and has the below guarantee:
    \begin{itemize}
        \item If $G$ is a metric, the algorithm outputs \textbf{METRIC} with probability 1;
        \item If $G$ is $\epsilon$-far from a metric, the algorithm outputs \textbf{NON-METRIC} with probability at least 2/3.
    \end{itemize}
\end{thm}
\begin{proof}
    Since the algorithm always output \textbf{METRIC} when no violations to the triangle inequality is detected, the first guarantee follows. Suppose $G$ is $\epsilon$-far from a metric. If there are at least $\epsilon^{1.1}n$ vertices participating in more than $n^{4/3}/4$ bad triangles, the first half of the algorithm, procedure HighDegreeDetection, finds a bad triangle and outputs \textbf{NON-METRIC} with probability at least 5/6. If there are less than $\epsilon^{1.1}n$ vertices participating in more than $n^{4/3}/4$ bad triangles, with probability at least 5/6 at least one bad triangle appears in the clique formed by the $s$ vertex samples in the second half of the algorithm, procedure BadTriangleDetection, and the algorithm outputs \textbf{NON-METRIC}. By union bound, the second guarantee follows.

    Procedure HighDegreeDetection samples $O(1/\epsilon^{1.1})$ vertices and $O(n^{2/3})$ edges and make pairwise queries between each $(vertex, edge)$ tuple. Procedure BadTriangleDetection samples $O(n^{1/3}/\epsilon)$ vertices and make $O(n^{2/3}/\epsilon^2)$ queries between each pair of vertices. Hence, the query complexity of Metric Testing is bounded by $O(n^{2/3}/\epsilon^2)$.
\end{proof}











\subsection{Query complexity lower bound for one-sided error testing algorithm}

We now show here a construction of distance matrix such that, once corruption parameter $\epsilon$ is set to be less than $n^{-\nu(n)}$ where $\nu(n)=\frac{\log\log\log(n)+4}{\log\log(n)}$ is a $o(1)$ function of $n$, then a cubic root dependence on $n$ appears in any one-sided error tester. Formally, the main result is as follows.
\begin{thm}
    Suppose $\epsilon\leq n^{-\nu(n)}$ where $\nu(n)=\frac{\log\log\log(n)+4}{\log\log(n)}$, then any one-sided error testing algorithm needs to make $\Omega(n^{1/3+\nu(n)/3})$ queries to decide whether a distance matrix is a metric or not in the worst case. For non-adaptive algorithm, it needs to make $\Omega(n^{2/3+2\nu(n)/3})$ queries.
\end{thm}

The construction follows closely to the Behrend graph construction used in~\cite{AKKR08} for showing the hardness of testing triangle-freeness. Their idea is to construct a graph with many edge-disjoint triangles, such that even an algorithm hits an edge, with low probability it can find the other two edges which form a triangle with the current edge. The technique used in their argument is to construct a Cayley graph using a Salem-Spencer set, or a 3-arithmetic-progression-free set, with large cardinality. Here, we re-use the Salem-Spencer set they construct and add more edges and weights to make the graph a clique.

\begin{lemma}\label{3APFreeSet}
    There exists a set $X\subseteq[n]$ with size at least $n^{1-\nu(n)}$ where $\nu(n)=\frac{\log\log\log(n)+4}{\log\log(n)}$ such that for all $x,y,z\in X$, if $x+z\equiv 2y\pmod{n}$, then $x=y=z$.\qed
\end{lemma}
\begin{lemma}\label{behrendGraph}
    Let $X$ be a 3-AP-free subset of $[n]$ in \hyperref[3APFreeSet]{Lemma~\ref*{3APFreeSet}}. Suppose $G'$ is a graph with vertex set $A\cup B\cup C$ where $A,B,C$ are three disjoint sets of $n$ vertices. Suppose for each of $A,B,C$, the vertices are labelled from $a_1$ to $a_n$, $b_1$ to $b_n$, and $c_1$ to $c_n$ respectively. The edges $E'$ in $G'$ are create following the protocols:
    \begin{itemize}
        \item $\forall a_i\in A,b_j\in B$, $(a_i,b_j)\in E'$ if and only if $\exists \,x\in X,j-i\equiv x\pmod{n}$;
        \item $\forall b_i\in B, c_j\in C$, $(b_i,c_j)\in E'$ if and only if $\exists \,x\in X,j-i\equiv x\pmod{n}$;
        \item $\forall a_i\in A,c_j\in C$, $(a_i,c_j)\in E'$ if and only if $\exists \,x\in X,j-i\equiv 2x\pmod{n}$.
    \end{itemize}
    Then, there are $3n|X|$ edges and $n|X|$ triangles in $G'$, all triangles are edge-disjoint.\qed
\end{lemma}
The construction of a large 3-AP-free set in \hyperref[3APFreeSet]{Lemma~\ref*{3APFreeSet}} could be found in~\cite{AKKR08}. The property that all triangles in the graph $G'$ in \hyperref[behrendGraph]{Lemma~\ref*{behrendGraph}} are edge-disjoint follows directly from the property of 3-AP-free set $X$.

Building on this graph construction, we provide below a distance matrix derived from a weighted clique, such that a large amount of edges have to be modified in order for the graph to obey triangle inequalities. The main theorem then follows from the below lemma.

\begin{lemma}\label{behrendGraphMatrix}
    Let $X$ be a 3-AP-free subset of $[n]$ as constructed in \hyperref[3APFreeSet]{Lemma~\ref*{3APFreeSet}}. Suppose $G$ is a clique graph with vertex set $A\cup B\cup C$ where $A,B,C$ are three disjoint sets with vertices labelling from $a_1$ to $a_n$, $b_1$ to $b_n$, and $c_1$ to $c_n$ respectively. Let $w:(A\cup B\cup C)\times (A\cup B\cup C)\ra\mathbb{R}^{>0}$ be an edge weight assignment defined as followed.
    \begin{itemize}
        \item $\forall a_i\in A,b_j\in B$, $w(a_i,b_j)=1$ if and only if $\exists\, x\in X,j-i\equiv x\pmod{n}$; $w(a_i,b_j)=2$ otherwise;
        \item $\forall b_i\in B, c_j\in C$, $w(b_i,c_j)=2$ if and only if $\exists\, x\in X,j-i\equiv x\pmod{n}$; $w(b_i,c_j)=3$ otherwise;
        \item $\forall a_i\in A,c_j\in C$, $w(a_i,c_j)=4$ if and only if $\exists\, x\in X,j-i\equiv 2x\pmod{n}$; $w(a_i,c_j)=2$ otherwise.
        \item for any pair of vertices $(x_i,y_j)$ in the same set $A,B,$ or $C$, $w(x_i,y_j)=2$.
    \end{itemize}
    Let $\psi:[3n]\ra A\cup B \cup C$ be any bijective map from points in $[3n]$ to vertices in $G.$ Let $M$ be a $3n\times 3n$ matrix, and set matrix entry $M(i,j)$ to be $w(\psi(i),\psi(j))$. Then, $2n|X|$ entries in $M$ have to be modified for $M$ to be a metric. Moreover, any one-sided error algorithm testing the metric property of $M$ by querying pairwise distances have to make $\Omega(n^{1/3+\nu(n)/3})$ queries to detect a violation to triangle inequality. For non-adaptive algorithms, $\Omega(n^{2/3+2\nu(n)/3})$ queries are needed to detect a violation.
\end{lemma}
\begin{proof}
    The claim in the lemma implies that $M$ is $\frac{|X|}{n}$-far from the metric property. That is, at least $|X|n$ entries need to be modified for $M$ to be a metric. Using the construction of 3-AP-free set in~\cite{AKKR08}, $M$ is $n^{-\nu(n)}$-far from the metric property.

    First, notice that all edge weights in $G$ are in $\{1,2,3,4\},$ meaning that the only 3-tuples possibly violating the triangle inequality have weights $(1,1,3),(1,1,4),(1,2,4)$. But the former two 3-tuples cannot appear as a 3-cycle in the graph $G$ as all edges with weight 1 are between vertex set $U$ and $V$. Hence, 3-cycles with edge weights $(1,2,4)$ are the only violations to the triangle inequality. It could then be verified that all 3-cycles with weights $(1,2,4)$ are exactly the triangles appeared in $G'$ constructed in \hyperref[behrendGraph]{Lemma~\ref*{behrendGraph}}. Thus, there are $n|X|$ edge-disjoint 3-cycles violating the triangle inequality. Each cycle $(i,j,k)$ corresponds to three matrix entries $M(i,j),M(i,k),M(j,k)$ according to the bijection $\psi$. Since all violating 3-cycles are edge-disjoint, each entry in $M$ is involved in at most one 3-tuples violating the triangle inequality. Moreover, since at least one entry in $M(i,j),M(i,k),M(j,k)$ has to be modified for the tuple $(i,j,k)$ to obey metric property, we need to modify at least one edge in each tuple. That is, at least $n|X|$ entries in $M$ has to be modified for $M$ to be a metric. In fact, exactly $n|X|$ modification suffices: simply modify all edges with weight 4 to 3. There are $n|X|$ such edges in $G$ corresponding to $2n|X|$ such entries in $M$.

    Now, we show the second argument in the lemma, that a non-adaptive algorithm needs to make $\Omega(n^{2/3+2\nu(n)/3})$ queries. First, continue the previous argument, 3-cycles with weights $(1,2,4)$ are the only evidence for the violation of triangle inequality, as longer cycles all obey the property. We show below that with $o(n^{2/3+2\nu(n)/3})$ queries, with high probability a non-adaptive algorithm detects no violation.

    Suppose a non-adaptive tester selects $k=o(n^{2/3+2\nu(n)/3})$ edges $\tilde{E}$ to find the violating cycles. The expected number of violating cycles among these edges, by the linearity of expectation, equals the probability that a random 3-cycle forms a violating cycle times the number of 3-cycles in $\tilde{E}$. This quantity is maximized when the queries $\tilde{E}$ form a clique. Therefore, with $k=o(n^{2/3+2\nu(n)/3})$ queries, in expectation $o(k^{3/2}\cdot|X|/n^2)=o(1)$ violating cycles could be found. Thus, a non-adaptive algorithm has to sample $\Omega(n^{2/3+2\nu(n)/3})$ edges before detecting a violation in expectation.
    
    For adaptive algorithm, suppose $\tilde{V}^t$ is a set of vertices that are appear in previous $t$ queries. When the $(t+1)^{th}$ query is made and it involves one or two vertices that are not in $\tilde{V}^t$, then all pairwise distances from $\tilde{V}$ to these new vertices are revealed to the tester. Therefore, at any point when $k$ vertices are being asked, the tester knows the clique formed by these $k$ vertices. Moreover, since all vertices are permuted uniformly, the tester cannot distinguish any two vertices which are not involved in previous queries, so the next new vertex the tester select is uniformly chosen. If only $k=o(n^{1/3+\nu(n)/3})$ vertices have been asked, the expected number of violation appearing in the sample is $o(1)$. Thus, an adaptive algorithm needs to make $\Omega(n^{1/3+\nu(n)/3})$ queries before seeing a violation in expectation.
\end{proof}





\subsection{Query complexity lower bound for two-sided error testing algorithm}

This section constructs a similar distance matrix $M'$ as in the previous section and shows that any two-sided error testing algorithm cannot do better than the one-sided error testing algorithm in terms of query complexity lower bound. The idea is to show that any two-sided error testing algorithm with query complexity $q(n)$ on $M'$ could be transformed into a one-sided error testing algorithm with query complexity $O(q(n))$ on distance matrix $M$ constructed previously.

In particular, we construct two graphs $G_g,G_b$ by ``doubling" the vertices in the graph $G$ constructed in \hyperref[behrendGraphMatrix]{Lemma~\ref*{behrendGraphMatrix}} in a way that any unbalanced 3-cycle in $G$ transforms into two unbalanced 3-cycles in $G_b$ while in $G_g$, it transforms into a balanced 6-cycles. For $G_b$, $\Omega(n|X|)$ edges need to be modified for the corresponding distance matrix to be a metric, while at the same time, $G_g$ corresponds to a metric. If a testing algorithm could distinguish between the two graphs $G_g,G_b$ using $q(n)$ queries, there exists an one-sided error testing algorithm for the metric property of graph $G$ with query complexity $O(q(n))$. The constructions for $G_g,G_b$ are given below. An immediate corollary is that, any non-adaptive two-sided error testing algorithm needs to make at least $\Omega(n^{2/3+2\nu(n)/3})$ queries to have a success probability at least 2/3.

\begin{lemma}
    Let $X$ be a 3-AP-free subset of $[n]$ as constructed in \hyperref[3APFreeSet]{Lemma~\ref*{3APFreeSet}}. Suppose $G_g,G_b$ are two cliques, each with vertex set $A\cup B\cup C$ where $A,B,C$ are three disjoint sets defined as $A=\{a_1,a_1',a_2,a_2',...,a_n,a_n'\}$, $B=\{b_1,b_1',...,b_n,b_n'\}$, and $C=\{c_1,c_1',...,c_n,c_n'\}$ respectively. Let $w_g,w_b:(A\cup B\cup C)\times (A\cup B\cup C)\ra\mathbb{R}^{>0}$ be two edge weight assignments, for $G_g,G_b$ respectively, defined as followed.
    \begin{itemize}
        \item $\forall x\in X,i\in[n],$ let $j=i+x,k=i+2x$, for edges between sets $A,B$, define $$w_b(a_i,b_j)=w_b(a_i',b_j')=w_g(a_i,b_j')=w_g(a_i',b_j)=1.$$ For other edges between $A,B$, define their weights to be 2. 
        
        For edges between $B,C$, define $$w_b(b_i,c_j)=w_b(b_i',c_j')=w_g(b_i,c_j')=w_g(b_i',c_j)=2,$$ For other edges between $B,C$, define their weights to be 3.
        
        for edges between $A,C$, define $$w_b(a_i,c_k)=w_b(a_i',c_k')=w_g(a_i,c_k')=w_g(a_i',c_k)=4,$$ For other edges between $A,C$, define their weights to be 2.
        
        \item For any pair of vertices $(x_i,y_j)$ in the same set $A,B,$ or $C$, $d(x_i,y_j)=2$.
    \end{itemize}
     Then, permute the vertex labels uniformly at random within each set $A,B,C$. Let $\psi:[6n]\ra A\cup B\cup C$ be any bijective map. Let $M_g,M_b$ be two $6n\times 6n$ matrices, and set matrix entry $M_g(i,j)$ to be $w_g(\psi(i),\psi(j))$, set matrix entry $M_b(i,j)$ to be $w_b(\psi(i),\psi(j))$. Then, both matrix $M_g$ and graph $G_g$ are metrics. Meanwhile, $2n|X|$ entries in $M_b$ have to be modified for $M_b$ to be a metric. With probability 1/2, matrix $M'$ is defined to be $M_g$, otherwise it is defined to be $M_b$. Any two-sided error tester with query complexity $q(n)$ on matrix $M'$ implies a one-sided error tester with query complexity $O(q(n))$ on matrix $M$ defined in Lemma~\ref{behrendGraphMatrix}.
\end{lemma}
\begin{proof}
    First, notice that the graphs $G_b,G_g$ are similar to the construction of $G$ in Lemma~\ref{behrendGraphMatrix}. The vertices of $G$ is duplicated. In $G_b$, the bad triangles in $G$ are also doubled: a bad triangle $(a,b,c)\in G$ corresponds to two bad triangles $(a,b,c),(a',b',c')\in G_b$. However, a bad triangle $(a,b,c)\in G$ corresponds to a 6-cycle in $G_g$, namely $(a,b',c,a',b,c')$. This 6-cycle has edge weights $(1,2,4,1,2,4)$ and so is a balanced cycle. By similar argument as in Lemma~\ref{behrendGraphMatrix}, $G_g$ is a metric as no triangle violates triangle inequality. As a contrast, there are exactly $2n|X|$ pair-wise disjoint bad triangles with weights $(1,2,4)$ in $G_b$. Hence, at least $2n|X|$ edges in $G_b$ needs to be modified for it to be a metric.

    Any two-sided error tester $T'$ that answers the question, is matrix $M'$ a metric or $\epsilon$-far from a metric for $\epsilon=n^{1-\nu(n)}$, with success probability at least 2/3 needs to distinguish matrices $G_b,G_g$ with probability at least 2/3. Then, there must exists an index $i\in[n]$ and $x\in X$ such that the tester queried at least one edge in $\{(a_i,b_{i+x}),(a_i,b_{i+x}'),(a_i',b_{i+x}),(a_i',b_{i+x}')\}$, at least one edge in $\{(b_i,c_{i+x}),(b_i,c_{i+x}'),(b_i',c_{i+x}),(b_i',c_{i+x}')\}$, and at least one edge in $\{(a_i,c_{i+2x}),(a_i,c_{i+2x}'),(a_i',c_{i+2x}),(a_i',c_{i+2x}')\}$. Otherwise, since the vertices are permuted uniformly, conditioned on the outcomes of the query, $M'=M_g$ or $M_b$ with equal probability. 

    Now, create another tester $T$ for matrix $M$ based on $T'$. Whenever $T'$ queries edge $(x,y),(x,y'),(x',y),$ or $(x',y')$, $T$ makes a query on edge $(x,y)\in G$. Since the tester $T'$ makes query on at least one edge in $\{(a_i,b_{i+x}),(a_i,b_{i+x}'),(a_i',b_{i+x}),(a_i',b_{i+x}')\}$, at least one edge in $\{(b_i,c_{i+x}),(b_i,c_{i+x}'),(b_i',c_{i+x}),(b_i',c_{i+x}')\}$, and at least one edge in $\{(a_i,c_{i+2x}),(a_i,c_{i+2x}'),(a_i',c_{i+2x}),(a_i',c_{i+2x}')\}$, the tester $T$ asks for weights of $(a_i,b_{i+x}),(b_{i+x},c_{i+2x}),$ and $(a_i,c_{i+2x})$. These three edges form a bad triangle in $G$, so $T$ immediately finds a violation in $G$. Hence, a tester on $M'$ with query complexity $q(n)$ that success with probability 2/3 implies the existence of another tester on $M$ with query complexity $O(q(n))$ with success probability at least 2/3.
\end{proof}


\section{Testing Ultrametric}\label{sec:ultra}

Results from the previous section shows that violations to triangle inequality are hard to detect. When the fraction of corruptions is small, then any non-adaptive tester needs to make $\Omega(n^{2/3+\nu(n)})$ queries to distinguish metric from a matrix that is far from having the metric property, where $\nu(n)=o(1)$. Even adaptive algorithm has a cubic root dependence on $n$ in the query complexity. This is because one change to the original metric (a ``corruption") might only ruin few triangles and hidden in most triangles. Even the tester samples this corrupted entry from the matrix, it cannot realize the entry is different from what it should be because the entries who form a violation to the triangle inequality along with this entry have not been sampled yet. Detecting a violation really boils down to sampling the very few 3-point-tuples which together show up as bad triangles, and it is hard for a tester to hit one of these $O(\epsilon)$ fraction of triangles. 

On the other hand, in this section, we show that violations to ultrametric is easy to detect. Recall that the ultrametric property imposes a very strict relationship on each three point tuple.
\begin{definition}[Ultrametric]
    A distance matrix $M\in \mathbb{R}^{n\times n}$ is an ultrametric if $M$ is a metric and the following condition holds.
    \begin{itemize}
        \item $M(i,j)\leq \max\{M(i,k),M(j,k)\}$ $\forall i,j,k\in[n]$.
    \end{itemize}
\end{definition}
This definition implies that among three points, knowing two pairwise distances might reveal the third distance. Hence, from the structural constraints imposed by the ultrametric property, one change in the ultrametric (a ``corruption") might ruin multiple triangles, who all are evidence that the given distance matrix is no longer an ultrametric. There exists a testing algorithm that picks up one of these evidences efficiently, namely with query complexity not depending on $n$.

More specifically, we present in this section a testing algorithm that, given query access to $M$, selects $O(\log(1/\epsilon)/\epsilon)$ points and decides whether $M$ is an ultrametric or $\epsilon$-far from an ultrametric with high success probability. In later sections, we also show that this bound is almost tight: any tester needs to sample $\Omega(1/\epsilon)$ points to before making an accurate decision.

In terms of query complexity, our algorithm makes pair-wise queries between the sampled points, achieving a query complexity of $\tilde{O}(1/\epsilon^2)$. We also constructs a distance matrix showing that any tester needs to make $\Omega(1/\epsilon^{4/3})$ queries to detect a violation.

The testing algorithm we provide in this section is the same as in~\cite{MD}. They achieved a sample complexity of $\tilde{O}(1/\epsilon^3)$ and a query complexity of $\tilde{O}(1/\epsilon^6)$. Our analysis, on the other hand, sheds light to the decaying speed of the sampled points revealing the corruptions and thus lower the sample and query complexity to $\tilde{O}(1/\epsilon)$ and $\tilde{O}(1/\epsilon^2)$, respectively. 

In particular, the testing algorithm has two phases, where it samples $\Omega(\log(1/\epsilon)/\epsilon)$ points in the first phase and another $\Omega(1/\epsilon)$ points in the second phase. In the first phase, the samples are used to build a skeleton tree. In the second phase, the skeleton tree constructed in the first phase is used to test the correctness of another set of points. The purpose of the skeleton tree constructed in the first phase is to impose plenty of structural constraints on the remaining points. In this way, the corruptions are no longer hidden; when some entries are corrupted from an utlrametric and one of the corruptions is sampled by our algorithm, our algorithm immediately recognizes this corruption because it forms a violation to the ultrametric property with the skeleton tree. The improvement of our query complexity is due to a careful analysis on how quickly the enlarging skeleton tree forms violations with more and more corrupted entries.

In the case that the given metric is indeed an ultrametric, the algorithm will not detect any corruptions and, as a result, output ``ULTRAMETRIC". If the given metric is $\epsilon$-far from being an ultrametric, we will show that the algorithm detects an error with high probability. Hence, in the following analysis, we assume that the given metric $M$ is $\epsilon$-far from an ultrametric. That is, at least $\epsilon n^2$ many entries inside the $n\times n$ matrix $M$ need to be modified so that $M$ becomes an ultrametric. The definition for a corrupted entry naturally arises.

\begin{definition}\label{ultracorrupt}
    Among the ultrametrics that are closest to $M$ in $\ell_0$ distance, we fix an ultrametric $M'$. Then an entry $M(i,j)$ is corrupted if $M(i,j)\neq M'(i,j).$
\end{definition}


\begin{definition} For a set of sampled points $U$, two points $a,b\notin U$ are in an equivalence class if and only if $M(a,x)=M(b,x)$ for all $x\in U$.
\end{definition}

We borrow the definition of equivalence class from~\cite{MD}. The distance between two points $a,b$ in different equivalent classes can be deduced from the skeleton tree. This is because, by the definition of equivalence classes, there must be a point $u \in U$ such that $M(u,a) \not= M(u,b)$ and thus $M(a,b)$ must be equal to
$\max (M(u,a), M(u,b))$. Hence, if the deduced distance is different from $M(a,b)$, then we have detected a violation of the ultrametric property at tuple $(a,b,u)$.

On the other hand, we cannot deduce the distance between unsampled $a,b$ if they fall into the same equivalence class. Imagine sorting the rows and columns of the given distance matrix $M$ in the way that points in the same equivalence class are put together. These entries form a block diagonal matrix. In consequence, each off-diagonal entry represents the distance between some two points in different equivalence classes.

Building onto the definition of equivalence classes, each time a new point $y$ is sampled and added into $U$, the new partition formed by $U$ is a refinement of the old partition. Therefore, sampling a new point can be viewed as moving some entries from diagonal blocks to off-diagonal blocks.

Now we consider a diagonal block $B$. Points included in this block have the same distance to the existing points in $U$. Even though we cannot deduce the pairwise distance between points in $B$, we have partial information about them. In particular, each entry $M(i,j)$ in $B$ is no larger than $M(i,u)=M(j,u)$ for all $u\in U$. If some entry $M(i,j)$ violates this constraint and is sampled, the algorithm will spot this corruption as it forms a violation to the ultrametric property with some point $u\in U$ in the current sample set. Conditioned on the current sample set, we call this kind of corruption an ``easy-to-detect-corruption".

\begin{definition}
    For an equivalence class $B$ generated by a set of samples $U$, an entry $M(i,j)$ in $B$ is an easy-to-detect-corruption if for some $u\in U$, $M(i,u)=M(j,u)<M(i,j).$
\end{definition}

The set of current samples $U$ imposes an upper bound to the possible values in $B$ which is $\min_{u\in U} M(u,x),$ for any $x\in B$. An entry in $B$ is larger than this threshold if and only if it is an easy-to-detect-corruption.

In contrast, a corruption can be ``hard to detect": For example, when there are three points $i,j,k$ in a block such that $M(i,j),M(i,k),M(j,k)$ are three different values, all less than $\min_{u\in U} M(i,u)$. 

Focusing on a single diagonal block $B$ with $\beta n$ many points, if the number of easy-to-detect-corruptions in $B$ is larger than $(\beta n)^2/2$, we call this block a ``bad block", since once we sample an entry from this block, with probability 1/2 it is a corruption, and we can recognize it immediately using $U$. On the other hand, if the \textit{total} number of corruptions in $B$ is smaller than $\beta \cdot\epsilon n^2/2$, we call this block ``good block". That is, a block with $\beta$ fraction of points but less than $\beta/2$ fraction of corruptions. Notice that a block can be good and bad at the same time. If a block is neither good nor bad, we call them active blocks.

In summary, the blocks are categorized into 3 categories, based on the number of corruptions. 
\begin{description}
    \item[Bad blocks] A block with $\beta n$ many points and more than $(\beta n)^2/2$ easy-to-detect-corruptions.
    \item[Good blocks] A block with $\beta n$ many points and less than $\beta\cdot\epsilon n^2/2$ total corruptions. 
    \item[Active blocks] We call a block ``active" if it is neither good or bad. 
\end{description}

Intuitively, if there are many bad blocks, then it implies there are many easy-to-detect-corruptions. The algorithm samples entries uniformly and use $U$ to recognize these corruptions. On the other hand, if there are many good blocks, then that means $\Omega(\epsilon n^2)$ corruptions must lie off-diagonal. As a result, they can also be easily detected with $U$ in the second phase of the algorithm. 

Formally, suppose at some stage with the current sample $U$, the total number of entries in the active blocks is less than $\epsilon n^2/4$. Since the good blocks contain at most $\epsilon n^2/2$ many corruptions, at least $\epsilon n^2/4$ corruptions stay in the bad blocks or off-diagonal. Moreover, since more than half of the entries in the bad blocks are easy-to-detect-corruptions, among the corruptions either staying in the bad blocks or off-diagonal, at least half of them are either easy-to-detect or off-diagonal. Therefore, we claim that the number of off-diagonal corruptions plus the number of on-diagonal easy-to-detect-corruptions is at least $\epsilon n^2/8$.

\begin{lemma}\label{lem:lowActiveMeansEasyToDetect}
    At some stage when the total number of active entries is less than $\epsilon n^2/4$, there are at least $\epsilon n^2/8$ corruptions being either off-diagonal or on-diagonal but easy-to-detect. \qed
\end{lemma}

The above claim shows that when there are not so many entries in the active blocks, the corruptions can be easily recognized with the samples $U$. So what if there are many entries in the active blocks? Below, we show that when sampling a point from an active block, we expect to move a lot of entries from on-diagonal to off-diagonal. As a result, the total number of active entries decrease quickly.

Suppose some on-diagonal block $B_i$ is active. We show that if a point $x$ is sampled from this block, then a large number of ``separations" is created in expectation, which explains the name of this category. Here, a separation happens when a pair of points $a,b$ in the same equivalence class under a set of samples $U$ is separated into two classes with respect to the new set of samples $U\cup\{x\}$. As a consequence, the entry $(a,b)$ moved from on-diagonal to off-diagonal. The following lemma states this claim formally. The main idea of the proof is that, since the block is not good, there are many corruptions. It implies that the ``entropy" within the block is large, i.e., the block is far from having all entries the same value. Then, picking a point $x$ from the block will divide the points in $B$ into equivalence classes according to their values on the row corresponding to $x$. Namely, points with same the value on the row corresponding to $x$ are put into the same equivalence class.

\begin{lemma}\label{active} Suppose a block $B$ with $\beta n$ points is neither good nor bad. If a point is sampled from $B$, we expect to move at least $\beta\cdot\epsilon n^2/16$ entries from on-diagonal $B$ to off-diagonal.
\end{lemma}
\begin{proof}
By definition of good and bad, $B$ has more than $\beta\cdot\epsilon n^2/2$ corruptions and less than $(\beta n)^2/2$ easy-to-detect-corruptions. Consider only the entries that are either un-corrupted or corrupted but not easy-to-detect. Suppose the set of values these entries take on is $\{v_1,v_2,...,v_k\},$ and further suppose $v_1$ is the value that most entries take on. Suppose $\{v_{k+1},...,v_{l}\}$ is the set of values the easy-to-detect-corrupted entries take on. Following the definition of easy-to-detect-corruptions, any value in $\{v_{k+1},...,v_{l}\}$ is larger than any value in $\{v_1,v_2,...,v_k\},$ so $\{v_1,...,v_l\}$ is a set of non-repetitive values. Let $r_i$ to denote the number of entries taking on value $v_i$ in the block $B$. Hence, $\sum_{i=1}^lr_i=(\beta n)^2.$ The assumption indicates that $r_1\geq r_i,\forall i\in\{2,...,k\},$ and $\sum_{i=k+1}^lr_i$, being the number of easy-to-detect-corruptions, is no larger than $(\beta n)^2/2$.


Now, we calculate the expected number of separations when we sample a point $x$ from $B$. In the row of $B$ that corresponds to point $x$, suppose there are $r_i^{(x)}$ entries whose values are $v_i$. Then, once $x$ is sampled, the number of separations created is $\sum_{i=1}^lr_i^{(x)}(\beta n-r_i^{(x)})/2.$ Summing over all points in $B$, the expected number of separations created when a point is selected from $b$ is $\frac{1}{\beta n}\sum_{x\in B}\sum_{i=1}^lr_i^{(x)}(\beta n-r_i^{(x)})/2=\frac{1}{2\beta n}\sum_{i=1}^l\sum_{x\in B}r_i^{(x)}(\beta n-r_i^{(x)}).$

To find a lower bound for the above quantity, we first consider the number of separations one value $v_i$ generated. Imagine we have a graph with $\beta n$ vertices, and two vertices $x,y$ are connected by an edge if and only if the entry $(x,y)$ in $B$ equals $v_i$. Then there are $r_i/2$ edges in this graph, and the degree of a vertex $x$ is $r_i^{(x)}$. Thus, $\sum_{x\in B}r_i^{(x)}(\beta n-r_i^{(x)})=\beta n\cdot\sum_{x\in B}r_i^{(x)}-\sum_{x\in B}(r_i^{(x)})^2=\beta n\cdot r_i-\sum_{x\in B}(r_i^{(x)})^2$. De Caen~\cite{D} gives an upper bound on the sum of squared degrees, that $\sum_{x\in B}(r_i^{(x)})^2\leq E({2E}/({V-1})+V-2)\approx{r_i^2}/{(2\beta n)}+r_i\cdot\beta n/2$. On the other hand, since $r_1\geq r_i,\forall i\in\{2,...,k\},$ an upper bound for $\sum_{i=1}^lr_i^2$ is $(\sum_{i=k+1}^lr_i)^2+((\beta n)^2-\sum_{i=k+1}^lr_i)r_1$, where, recall that, the quantity $\sum_{i=k+1}^lr_i$ is the total number of easy-to-detect corruptions. To sum up, the expected number of separations is at least 
\begin{align*}
    &\frac{1}{2\beta n}\sum_{i=1}^l\sum_{x\in B}r_i^{(x)}(\beta n-r_i^{(x)})
    \\\geq&\frac{1}{2\beta n}\sum_{i=1}^lr_i\cdot\beta n-\frac{r_i^2}{2\beta n}-r_i\cdot\beta n/2
    \\=&\frac{1}{2\beta n}(\beta n)^3-\frac{1}{4(\beta n)^2}\sum_{i=1}^lr_i^2-\frac{(\beta n)^2}{4}
    \\\geq&\frac{(\beta n)^2}{4}-\frac{1}{4(\beta n)^2}((\sum_{i=k+1}^lr_i)^2-r_1\cdot\sum_{i=k+1}^lr_i)-\frac{r_1}{4}.
\end{align*}
% D. de Caen, An upper bound on the sum of squares of degrees in a graph
To further bound this quantity, we consider two cases for the size of $r_1$, or the number of entries taking on value $v_1$.
\begin{itemize}
    \item CASE $r_1\leq (\beta n)^2/2:$ Following the assumption that block $B$ is not bad, $\sum_{i=k+1}^lr_i$, being the number of easy-to-detect corruptions, shall not exceed $(\beta n)^2/2$. Thus, the above expected number of separations is at least $(\beta n)^2/4-(\beta n)^4/(16(\beta n)^2)-r_1/4=3(\beta n)^2/16-r_1/4$. As a consequence, $8\times\mathbb{E}_{x\in B}[\text{separations created by } x]\geq(\beta n)^2-r_1$.
    \item CASE $r_1>(\beta n)^2/2$: Notice that $\sum_{i=k+1}^lr_i\leq (\beta n)^2-r_1<(\beta n)^2/2$. In this case, the above expected number of separations is minimized when $\sum_{i=k+1}^lr_i$ is 0 or $(\beta n)^2-r_1$ by convexity, corresponding to $\mathbb{E}_{x\in B}[\text{separations created by } x]\geq\max\{(\beta n)^2/4-r_1/4,r_1/2\}$. Again, it implies that $8\times\mathbb{E}_{x\in B}[\text{separations created by } x]\geq(\beta n)^2-r_1$.
\end{itemize}

Now we switch gear and ponder upon the implications of corruptions. Notice that, if we modify all values in $\{v_2,\ldots,v_l\}$ to $v_1$, $B$ will become an all-$v_1$ matrix, which is an ultrametric. This suggest the block $B$ is $(\sum_{i=2}^lr_i)$-close to an ultrametric. Therefore, the ultrametric $M'$ we fixed in \hyperref[ultracorrupt]{Definition~\ref*{ultracorrupt}} shouldn't be $(\sum_{i=2}^lr_i)$-far from $M$ in this block $B$. Otherwise, there exists an ultrametric $M''$ which is closer to $M$ in terms of $\ell$-0 distance. (This $M''$ will be the same as $M'$ except that the block $B$ in $M''$ is an all-$v_1$ matrix.) Therefore, we claim that the number of corruptions in $B$ of our metric $M$, which is defined to be the number of entries that $M$ and $M'$ disagree on, should not exceed $\sum_{i=2}^lr_i=(\beta n)^2-r_1$. %This quantity, as shown above, is approximately 8 times the lower bound of the expected number of separations. 

Since block $B$ is not good, there are at least $\beta \cdot\epsilon n^2/2$ corruptions in the block. As a summary for the above inequalities, we have $$8\times \mathbb{E}_{x\in B}[\text{separations created by } x]\geq (\beta n)^2-r_1\geq \#\text{ of corruptions in }B\geq \beta\cdot\epsilon n^2/2.$$
Therefore, when a point is sampled from $B$, we expect to create $\beta \cdot\epsilon n^2/16$ separations, or equivalently, we expect to move $\beta \cdot\epsilon n^2/16$ entries from on-diagonal $B$ to off-diagonal.


\end{proof}

At this moment, we know what happen to one active block when a point is sampled from that block. Now, we zoom out from the picture and analyze how this decrease of the on-diagonal active entries compare to the total number of active entries. 

\begin{lemma}
    Suppose at some stage the algorithm have sampled $t$ points from the active blocks. There are a total of $x_t$ entries in the active blocks, represented by $\alpha_t n$ many points. After sampling the $(t+1)^{st}$ point from the active blocks, we expect to have no more than $x_t\cdot\exp(-\frac{\epsilon}{16\alpha_t})$ entries staying in the active blocks. 
\end{lemma}
\begin{proof}
    This statement follows from the previous lemma. Suppose the block $B_i$ with $\beta_in$ points is active. A point is chosen from this block with probability $\beta_i$, and, as a result, at least $\beta_i\cdot\epsilon n^2/16$ entries are being relocated to off-diagonal places in expectation. Thus, conditioned on some point is sampled from the active blocks, the expected amount of decrease on the on-diagonal entries is at least $$\frac{\sum_{i\text{ is active}}\beta_i^2\cdot \epsilon n^2/16}{\alpha_t},$$ so we have $$\mathbb{E}[x_{t+1}|x_t,\alpha_t]\leq x_t-\frac{\sum_{i\text{ is active}}\beta_i^2\cdot \epsilon n^2/16}{\alpha_t}$$ On the other hand, the total amount of entries at time $t$ in the active blocks is $$x_t=\sum_{i\text{ is active}}(\beta_in)^2.$$ Hence, after the $(t+1)^{st}$ point is selected from the active blocks, we expect to have $\mathbb{E}[x_{t+1}|x_t,\alpha_t]\leq x_t-x_t\cdot\frac{\epsilon}{16\alpha_t}\leq x_t\cdot\exp(-\frac{\epsilon}{16\alpha_t})$ entries staying in the active blocks, on the diagonal.
\end{proof}

\begin{corollary} Again, let $x_t$ and $\alpha_tn$ to denote the number of entries and points in the active blocks after $t$ points have been sampled from the active blocks. Then
$\mathbb{E}[\log(x_{t+1})]\leq \mathbb{E}[\log(x_t)]-\mathbb{E}[\frac{\epsilon}{16\alpha_t}].$
\end{corollary}
\begin{proof}
    $\mathbb{E}[\log(x_{t+1})]=\mathbb{E}[\mathbb{E}[\log(x_{t+1})|x_t,\alpha_t]]\leq\mathbb{E}[\log(\mathbb{E}[x_{t+1}|x_t,\alpha_t])]\leq\mathbb{E}[\log(x_t)-\frac{\epsilon}{16\alpha_t})]
    =\mathbb{E}[\log(x_t)]-\mathbb{E}[\frac{\epsilon}{16\alpha_t}],$ where the first inequality follows from Jensen's inequality and the second inequality follows from the previous lemma.
\end{proof}


We start with $n^2$ on-diagonal active entries, and stop sampling when the amount of active entries to be so small that the corruptions are either off-diagonal or on-diagonal but easy to be detected. Suppose we increment time by one whenever a sampled point is from the active block. Following the previous corollary, by induction, we have $$\mathbb{E}[\log(x_T)]\leq\mathbb{E}[\log(x_{0})]-\sum_{t=0}^{T-1}\mathbb{E}[\frac{\epsilon}{16\alpha_t}]=\log(n^2)-\sum_{t=0}^{T-1}\mathbb{E}[\frac{\epsilon}{16\alpha_t}].$$ We want, in the end, the number of active entries fall under $\epsilon n^2/48$ in expectation. That is, we need $T$ such that $\sum_{t=0}^{T-1}\mathbb{E}[\frac{\epsilon}{16\alpha_t}]\geq\log(\frac{48}{\epsilon})$. 

On the other hand, conditioned on having $\alpha_tn$ points in the active blocks at time $t$, we expect to sample $1/\alpha_t$ points to hit the $(t+1)^{st}$ active point and increase time to $t+1$. Thus, to reach time $T$, we expect to sample $\sum_{t=1}^{T-1}\mathbb{E}[\frac{1}{\alpha_t}]$ points. Since $\sum_{t=0}^{T-1}\mathbb{E}[\frac{\epsilon}{16\alpha_t}]\geq\log(\frac{48}{\epsilon})$, after sampling $16\log(48/\epsilon)/\epsilon$ points, the number of active entries is reduced to $\epsilon n^2/24$ in expectation. 

\begin{lemma}
    Suppose the algorithm samples $192\cdot \log(48/\epsilon)/\epsilon$ points at random and did not detect an error after querying their pairwise distance. Then with probability larger than 5/6, the number of on-diagonal active entries is less then $\epsilon n^2/4$.
\end{lemma}
\begin{proof}
    Above analysis has shown that the algorithm needs to sample no more than $16\cdot \log(48/\epsilon)/\epsilon$ points in expectation to reach the final stage $T$. Moreover, at final stage $T$, in expectation there are no more than $\epsilon n^2/48$ active entries. Hence, with probability 11/12, $192\cdot \log(48/\epsilon)/\epsilon$ points suffice to bring us to the final stage, and with probability 11/12, no more than $\epsilon n^2/4$ active entries are left in the final stage. The statement follows from an union bound.
\end{proof}

In summary, the first phase of the algorithm randomly samples $\tilde O(1/\epsilon)$ points to make sure there are at least $\Omega(\epsilon n^2)$ off-diagonal or on diagonal but easy to detect corruptions.

\begin{lemma}\label{success prob bound}
    Suppose after sampling a set $U$ with $192\cdot \log(48/\epsilon)/\epsilon$ points at random and querying the distance between these points, the algorithm has not detected any violation. Then, the algorithm samples another set $P$ of $16/\epsilon$ entries at random. For each entry $(i,j)\in P$, the algorithm queries $M(i,j)$ and $M(i,u),M(j,u)$ for all $u\in U$, and see if there is any violation to the ultrametric property. Then, with probability larger than 2/3, the algorithm detects a violation.
\end{lemma}
\begin{proof}
    The above lemma showed that after sampling $192\cdot \log(48/\epsilon)/\epsilon$ points in the first phase, with probability larger than 5/6, the total number of active entries is below $\epsilon n^2/4$. \hyperref[lem:lowActiveMeansEasyToDetect]{Lemma~\ref*{lem:lowActiveMeansEasyToDetect}} showed that there are at least $\epsilon n^2/8$ entries that are either off-diagonal corruptions or on-diagonal but easy-to-detect corruptions. Either off-diagonal corruptions or on-diagonal easy-to-detect corruptions form a violation to the ultrametric property when adding the two points in that entry to $U$. Therefore, a random sampling on the entries of size $16/\epsilon$ hits a corruption with probability larger than $1-\exp(-2)>5/6,$ and the lemma follows from the union bound with the first phase success probability.
\end{proof}
We provide the pseudocode for the algorithm below. With Lemma~\ref{success prob bound}, we have the theorem for ultrametric testing.
\begin{thm}
    Algorithm~\ref{algo:ultra} takes in an input distance matrix $M\in\mathbb{R}^{n\times n}$, samples $O(\log(1/\epsilon)/\epsilon)$ points and has the below guarantee:
    \begin{itemize}
        \item If $M$ is an ultrametric, the algorithm outputs \textbf{ULTRAMETRIC} with probability 1;
        \item If $M$ is $\epsilon$-far from any ultrametric, the algorithm outputs \textbf{NON-ULTRAMETRIC} with probability at least 2/3.
    \end{itemize}
    \qed
\end{thm}
\begin{algorithm}
\caption{Ultrametric Testing}\label{algo:ultra}
\begin{algorithmic}
\Procedure{TestUltrametric}{$M$}
\State\Comment{$M\in \mathbb{R}^{n\times n}$ is a distance matrix on $n$ points}
\State $U\gets$ sample $192/\epsilon\cdot \log(48/\epsilon)$ points at random
\For{every three-point-tuple $(u,v,w) \in U$}
\If {$TestViolation(M,u,v,w)= $ FAIL}
\State\Return \{NON-ULTRAMETRIC\}
\EndIf
\EndFor
\State $P\gets$ sample $16/\epsilon$ pairs of points at random
\For{every three-point-tuple $(u,v,w) \in U\cup P$}
\If {$TestViolation(M,u,v,w)=$ FAIL}
\State\Return \{NON-ULTRAMETRIC\}
\EndIf
\EndFor
\State\Return ULTRAMETRIC

\EndProcedure

\Statex
\Procedure{TestViolation}{M,u,v,w}\Comment{$u,v,w$ are three points in the distance matrix $M$}
\If{$M(u,v)>\max\{M(u,w),M(v,w)\}$ \\or $M(u,w)>\max\{M(u,v),M(v,w)\}$ or $M(v,w)>\max\{M(u,v),M(u,w)\}$}
\State\Return FAIL
\EndIf
\State\Return PASS
\EndProcedure
\end{algorithmic}
\end{algorithm}










\section{Testing Tree Metric}\label{sec:tree} 
Recall that a distance metric is a tree metric if the points can be embedded to the leaves of a weighted tree graph. Also notice that ultrametric is a special kind of tree metric: each point corresponds to some leaf of the tree and every leaf has the same distance to the root node. Hence, the algorithm for testing tree metric has great similarity with the testing algorithm for ultrametric. Namely, it also divides into two phases, where the samples in the first phase are used to build a skeleton tree; the skeleton tree is then used in the second phase to verify the correctness of another set of samples.

If no violation to tree metric property is detected, the algorithm outputs ``YES". Hence, in the following analysis we assume the given metric is $\epsilon$-far from a tree metric, and the algorithm detects a violation with high probability and, as a result, outputs ``NO". Below, we formally define the tree metric and the corruptions inside $M$ which is analogous to the previous analysis on ultrametric testing.

\begin{definition}[Tree metric]
    A distance matrix $M\in \mathbb{R}^{n\times n}$ is a tree metric if $M$ is a metric and there exist a graph $G=(V,E)$ and an injection $\phi:[n]\ra V$ such that the following conditions hold.
    \begin{itemize}
        \item $G$ is non-negative, weighted, acyclic, undirected, and connected.
        \item $\forall i\in[n],\phi(i)$ is a vertex in $G$ with degree 1. That is, the image of $\phi$ are the leaves of $G$.
        \item $\forall i,j\in[n],M(i,j)=d(\phi(i),\phi(j)),$ where $d:V\times V\ra \mathbb{R}$ maps a pair of vertices to the length of the unique simple path connecting them in $G$.
    \end{itemize}
\end{definition}
 
\begin{definition}[Corruptions]
    Among the tree metrics that are the closest to $M$ in the $\ell$-0 distance, we fix an tree metric $M'$. An entry $M(i,j)$ is corrupted if $M(i,j)\neq M'(i,j).$
\end{definition}

The idea of analysis is similar to that of testing the ultrametric. The samples from the first phase are used to build a skeleton tree, which divides the remaining points into equivalence classes. When the skeleton tree grows, more structural constraints are imposed on the remaining points and the size of the equivalence classes shrink rapidly. Then, many entries which are corrupted form violations with the skeleton tree. The goal of the second phase is to sample one of such corrupted entries and test it against the skeleton tree. 

At first glance, the definition of tree metric is vague and hard to quantify as that of the ultrametric. Recall that a metric is an ultrametric if for every three-point-tuple, the larger two pairwise distances are the same. In fact, the tree embedding definition is equivalent to a four-point condition which emulates the three-point condition for ultrametric.

\begin{lemma} A metric $M$ on a set of points $S$ is consistent with a tree metric if and only if 
$$M(i,j)+M(k,l)\leq \max\{M(i,k)+M(j,l),\,M(i,l)+M(j,k)\},\,\forall i,j,k,l\in S.\qed$$
\end{lemma}
The condition is equivalently saying that, for all four-point tuple, if we define the value of a matching to be the sum of the two distances in this matching, then the max two matchings out of the three matchings should be the same. We call this the four-point condition or the four-point test. We will show that our testing algorithm detects a violation to the four-point test and realizes $M$ is not a tree metric with high probability.

In the previous analysis for ultrametric, after sampling a set $U$, two points are in the same equivalence class if for any point $u\in U$, the two points have the same distances to $u$. Such definition is motivated by the fact that, knowing their distances to points in $U$ does not provide much information to knowing the distance between the two points. On the other hand, the distance between two points in different equivalent classes can be easily deduced. Following the same motivation, we define the equivalences classes for tree metric.
\begin{definition}[Equivalence class]\label{treeequiv}
    For a set of sampled points $U$, two points $i,j$ are in the same equivalence class if and only if $M(i,u)-M(i,v)=M(j,u)-M(j,v)$ for all $u,v\in U$.
\end{definition}
The equation conveys the information that, out of the three matchings induced by $i,j,u,v$, the matching $M(i,u)+M(j,v)$ equals the matching $M(i,v)+M(j,u).$ In order for the four points to obey the four-point condition, we only need $M(i,j)+M(u,v)$ to be no more than this quantity. Even though we know $M(u,v)$ from the current samples, there is not much we can say about $M(i,j)$ other than an upper bound.

On the other hand, if two points $i,j$ fall into different classes, then $M(i,j)$ can be deduced exactly, since $M(i,j)=\max\{M(i,u)+M(j,v),M(i,v)+M(j,u)\}-M(u,v)$ if $M$ is a tree metric. Again, we sort the rows and columns of $M$ in the way that points in the same equivalence class are put together. Then, an equivalence class is represented as an on-diagonal block matrix.

There are, once more, easy-to-detect-corruptions and the non-easy-to-detect ones in an equivalence class. The above analysis gives hint on the definition.
\begin{definition}[Easy-to-detect corruptions]\label{treecorrupt}
    For an equivalence class $B$ generated by a set of samples $U$, an entry $M(i,j)$ in $B$ is an easy-to-detect corruption if for some $u,v\in U$, $M(i,j)+M(u,v)>M(i,u)+M(j,v)=M(i,v)+M(j,u).$
\end{definition}

Such corruption is easy to detect because the four-point-tuple $(i,j,u,v)$ violates the four-point condition. With this definition, we continue to use the bad, good, active categories to classify the blocks.
\begin{description}
    \item[Bad blocks] A block with $\beta n$ many points and more than $(\beta n)^2/2$ easy-to-detect-corruptions.
    \item[Good blocks] A block with $\beta n$ many points and less than $\beta\cdot\epsilon n^2/2$ total corruptions. 
    \item[Active blocks] We call a block ``active" if it is neither good or bad.
\end{description}

With the same argument as in the ultrametric testing analysis, if after sampling a set of points $U$, there are no more than $\epsilon n^2/4$ many entries in the active block, then there are at least $\epsilon n^2/8$ many corruptions either off-diagonal or on-diagonal but easy to detect.

Thus, the intricate analysis falls to the case where most of the entries are in the active blocks. We want to show again that when a point is sampled from these active entries, the number of on-diagonal entries decreases rapidly. A result that resembles \hyperref[active]{Lemma~\ref*{active}} arises. When a point is sampled from an active block, many entries are moving from on-diagonal to off-diagonal. Recall that the main idea in the proof of \hyperref[active]{Lemma~\ref*{active}} is that, since there are many corruptions inside the block, the block must be far from having all entries the same value. Otherwise, with many entries being the same, the block is close to an ultrametric which contradicts the fact that it contains many corruptions. When we sample a row from this block, entries that have different values are separated into different classes, so we expect many separations are created once we sample a point from this block. There is a slight difference in the tree metric case. When a point $x$ is being sampled from an active block, how the rest points in this block are divided into different classes is no longer according to their distances to $x$, but according to the difference between their distance to $x$ and their distance to some $u\in U$. This is due to how we define equivalence classes in \hyperref[treeequiv]{Definition~\ref*{treeequiv}}. Thus, after ``masking" the block with some distance matrix, we are able to re-use the same argument as before to prove the below lemma. 

With the following claim, we argue that the number of active entries decreases rapidly. In consequence, with few points sampled from the active blocks, the total number of active entries can be reduced to $\epsilon n^2/4$.

\begin{lemma}
    Suppose a block $B$ with $\beta n$ points is neither good nor bad. If a point is sampled from $B$, we expect to move at least $\beta\cdot \epsilon n^2/16$ entries from on-diagonal to off-diagonal.
\end{lemma}
\begin{proof}
    Suppose the $(i,j)$ entry of block $B$ gives the distance $M(x_i,x_j)$ between points $x_i$ and $x_j$. We fix a sampled point $u\in U$, and define a $\beta n\times \beta n$ masking matrix $\mathrm{MASK}$ where the $(i,j)$ entry of $\mathrm{MASK}$ equals $M(u,x_i)+M(u,x_j)$. That is,
\[
\renewcommand\arraystretch{1.3}
B=\mleft[
\begin{array}{cccc}
  M(x_1,x_1) & M(x_1,x_2) &\cdots &M(x_1,x_{\beta n})\\
   M(x_2,x_1) & M(x_2,x_2) &\cdots &M(x_2,x_{\beta n})\\
   M(x_3,x_1)& M(x_3,x_2) &\cdots &M(x_3,x_{\beta n})\\
  
  \vdots & \vdots & \ddots  &\vdots\\
   M(x_{\beta n},x_1) & M(x_{\beta n},x_2)  &\cdots &M(x_{\beta n},x_{\beta n})\\
\end{array}
\mright]
,
\]
\[
\renewcommand\arraystretch{1.3}
\mathrm{MASK}=\mleft[
\begin{array}{cccc}
  M(u,x_1)+M(u,x_1) & M(u,x_2)+M(u,x_1)  &\cdots &M(u,x_{\beta n})+M(u,x_1)\\
   M(u,x_1)+M(u,x_2) & M(u,x_2)+M(u,x_2)  &\cdots &M(u,x_{\beta n})+M(u,x_2)\\
   M(u,x_1)+M(u,x_3) & M(u,x_2)+M(u,x_3)  &\cdots &M(u,x_{\beta n})+M(u,x_3)\\
  
  \vdots & \vdots & \ddots  &\vdots\\
   M(u,x_1)+M(u,x_{\beta n}) & M(u,x_2)+M(u,x_{\beta n})  &\cdots &M(u,x_{\beta n})+M(u,x_{\beta n})\\
\end{array}
\mright]
.
\]
\hyperref[active]{Lemma~\ref*{active}} considers the values in the block matrix $B$. Here, instead, we consider the values in the square matrix $(B-\mathrm{MASK})$. The motivation is that, when we sample some point $x_i$ from the block $B$, other points in $B$ are partitioned according to the values in the $i^{th}$ row of $(B-\mathrm{MASK})$. In particular, for points $a,b$, 
\begin{align*}
&a,b\text{ are separated into two equivalance classes according to }U\cup\{x_i\}\\
\Leftrightarrow \,& M(x_i,a)+M(w,b)\neq M(w,a)+M(x_i,b)\text{ for some }w\in U\\
&\text{(definition of equivalence classes) }\\
\Leftrightarrow\,&M(x_i,a)+M(w,b)+M(u,b)\neq M(w,a)+M(x_i,b)+M(u,b)=M(w,b)+M(x_i,b)+M(u,a)\\
&\text{(equality follows from the fact that }a,b\text{ are in the same equivalence class under }U)\\
\Leftrightarrow\,&M(x_i,a)+M(u,b)\neq M(x_i,b)+M(u,a)\\
\Leftrightarrow \,&M(x_i,a)-M(u,x_i)-M(u,a)\neq M(x_i,b)-M(u,x_i)-M(u,b)\\
\Leftrightarrow \,&\text{ the }(x_i,a)\text{ and }(x_i,b)\text{ entry of the matrix }B-\mathrm{MASK}\text{ are different.}
\end{align*}

Among the entries that are either un-corrupted or corrupted but not easy-to-detect in $B$, suppose the set of the values these entries take on in $(B-\mathrm{MASK})$ is $V=\{v_1,v_2,...,v_k\}$, and further suppose $v_1$ is the value that most entries take on. Suppose $V'=\{v_{k+1},...,v_{l}\}$ is the set of values the easy-to-detect-corrupted entries in $B$ take on in the matrix $(B-\mathrm{MASK})$. We first show that any value in $V'$ is larger then any value in $V$, so as a result $\{v_1,...,v_k,v_{k+1},...,v_l\}$ is a set of non-repetitive values.
\begin{claim}
Suppose $v'\in V'$ and $v\in V$. Then $v'>v$.
\end{claim}
\begin{proof}
    Suppose the entry $(k,l)$ in $(B-\mathrm{MASK})$ takes on the value $v'$, which implies that $M(x_k,x_l)$ is an easy-to-detect-corruption and $v'=M(x_k,x_l)-M(u,x_k)-M(u,x_l)$. Suppose the entry $(i,j)$ in $(B-\mathrm{MASK})$ takes on the value $v$, which implies that $M(x_i,x_j)$ is either not a corruption, or it a corruption but not easy-to-detect. Moreover, $v=M(x_i,x_j)-M(u,x_i)-M(u,x_j)$. Since $M(x_k,x_l)$ is an easy-to-detect-corruption, by \hyperref[treecorrupt]{Definition~\ref*{treecorrupt}}, there exist some $a,b\in U$ such that $M(x_k,x_l)+M(a,b)>M(x_k,a)+M(x_l,b)$. On the other hand, as $M(x_i,x_j)$ is not an easy-to-detect-corruption, for the pair $a,b$, $M(x_i,x_j)+M(a,b)\leq M(x_i,a)+M(x_j,b).$

    Following the above facts, we have the inequalities
    \begin{align}
        v'=&M(x_k,x_l)-M(u,x_k)-M(u,x_l)\\
        >&M(x_k,a)+M(x_l,b)-M(a,b)-M(u,x_k)-M(u,x_l)\\
        =&M(x_i,x_j)+M(x_k,a)+M(x_l,b)-(M(a,b)+M(x_i,x_j))-M(u,x_k)-M(u,x_l)\\
        \geq&M(x_i,x_j)+M(x_k,a)+M(x_l,b)-(M(x_i,a)+M(x_j,b))-M(u,x_k)-M(u,x_l)\\
        =&M(x_i,x_j)+M(x_k,a)+M(x_l,b)-(M(x_i,a)+M(x_k,u))-(M(x_j,b)+M(x_l,u))\\
        =&M(x_i,x_j)+M(x_k,a)+M(x_l,b)-(M(x_i,u)+M(x_k,a))-(M(x_j,u)+M(x_l,b))\\
        =&M(x_i,x_j)-M(x_i,u)-M(x_j,u)=v,
    \end{align}
    where (2) and (4) follows from the above facts on easy-to-detect corruptions, (6) follows from the definition of $x_i,x_j,x_k,x_l$ being in the same equivalence class, and the rest equations are simply rearrangement of terms.
\end{proof}
    Now, by exactly the same argument as in \hyperref[active]{Lemma~\ref*{active}}, if we let $r_1$ to denote the number of entries taking on value $v_1$, then the expected number of separations after sampling a point from $B$ is at least $((\beta n)^2-r_1)/8$. What we left in this proof is to find a bound for $r_1$.

    Recall that in \hyperref[active]{Lemma~\ref*{active}}, we argued that if all values $v_2,...,v_l$ in $B$ are modified to be $v_1$, then the resulting matrix is an ultrametric. Same argument applies for $(B-\mathrm{MASK})$. If all values $\{v_2,...,v_l\}$ in this matrix are modified to be $v_1$, then after un-masking the modified matrix, we obtain a new block matrix $B'$ which is a tree metric and consistent with $U$. Hence, we only need to make $(\beta n)^2-r_1$ modifications to make this sub-matrix $B$ a tree-metric, implying that the number of corruptions in $B$ shall not exceed $(\beta n)^2-r_1$. Otherwise we can find a tree metric that is closer to $M$ in $\ell$-0 distance.
    \begin{claim}
        The $\beta n\times\beta n$ square matrix $B'$, which is the sum of all $v_1$ matrix and $\mathrm{MASK}$, is a tree metric. Moreover, if current samples $U$ form a tree and adding any one point from $\{x_1,...,x_{\beta n}\}$ in the block to $U$ will not generate violations, then adding all points $\{x_1,...,x_{\beta n}\}$ to $U$ according to the distances provided in $B'$ will not generate violations to the tree metric property.
    \end{claim}
    \begin{proof}
        Suppose $i,j,k,l$ are four points in the block. It is easy to check that all matchings have the same quantity, so they obey the four-point condition.

        Suppose $a,b$ are two points in $U$. The tuple $i,j,k,a$ obey the four-point condition because, $M(k,a)+B'(i,j)=M(k,a)+M(i,u)+M(j,u)+v_1=M(k,u)+M(i,a)+M(j,u)+v_1=M(i,a)+B'(k,j),$ and similarly, equals the third matching $M(j,a)+B'(i,k).$ The tuple $i,j,a,b$ obey the four-point condition because, $M(i,a)+M(j,b)=M(i,b)+M(j,a)$ by the definition of equivalence class, and $B'(i,j)+M(a,b)\leq M(i,a)+M(j,b).$ (The proof for this inequality shares the same flavor as the previous claim. It mainly follows from the fact that the value $v_1$ is taken by some entry in $(B-\mathrm{MASK})$ which correspond to some entry in $B$ that is not an easy-to-detect-corruption. )
    \end{proof}
    The above claim shows that we can modify $B$ within $(\beta n)^2-r_1$ entries to make it a tree metric that is consistent with $U$. Therefore, the number of corruptions in $B$ shall not exceed $(\beta n)^2-r_1$. Following the assumption that $B$ is not a good block, it contains more than $\beta\cdot\epsilon n^2/2$ corruptions. As before, we must have $$8\times\mathbb{E}_{x\in B}[\text{separations created by }x]\geq(\beta n)^2-r_1\geq \#\text{ of corruptions in }B\geq \beta\cdot\epsilon n^2/2,$$ so sampling a point from $B$ moves at least $\beta\cdot \epsilon n^2/16$ entries from on-diagonal to off-diagonal in expectation.
\end{proof}

Then, following the same stream of arguments as in the ultrametric case, we notice that the decrease in the number of active entries is rapid, as whenever a point is sampled from the active blocks, some considerable fraction of entries from active block are going from on-diagonal to off-diagonal. Suppose we
increment time by one whenever a sampled point is from the active block. The following two claims have exactly the same proof as before.

\begin{lemma}
    Suppose after sampling some points, we have sampled $t$ points from the active blocks. There are a total of $x_t$ entries in the active blocks, represented by $\alpha_t n$ many points. After sampling the $(t+1)^{st}$ point from the active blocks, we expect to have no more than $x_t\cdot\exp(-\frac{\epsilon}{16\alpha_t})$ entries staying in the active blocks. \qed
\end{lemma}
\begin{corollary} Again, let $x_t$ and $\alpha_tn$ to denote the number of entries and points in the active blocks after $t$ points have been sampled from the active blocks. Then
$\mathbb{E}[\log(x_{t+1})]\leq \mathbb{E}[\log(x_t)]-\mathbb{E}[\frac{\epsilon}{16\alpha_t}].$ \qed
\end{corollary}

As before, we start with $x_0=n^2$ on-diagonal active entries, and stop sampling after reaching a stage where $x_T\leq \epsilon n^2/4$. The argument resembles the ultrametric case, and it can be shown that in expectation, $16\log(4/\epsilon)/\epsilon$ samples suffice to reduce the active entries to $\epsilon n^2/4$. At this stage, $\epsilon n^2/8$ corruptions are either off-diagonal or on-diagonal but easy to be detected with $U$. Therefore, following exactly the same success probability analysis as in \hyperref[success prob bound]{Lemma~\ref{success prob bound}}, after sampling $\log(48/\epsilon)\cdot192/\epsilon$ points in the first phase and $16/\epsilon$ entries in the second phase uniformly at random, the testing algorithm detects a violation to the four-point condition with probability at least 2/3.


\begin{thm}
    Algorithm~\ref{algo:tree} takes in an input distance matrix $M\in\mathbb{R}^{n\times n}$, samples $O(\log(1/\epsilon)/\epsilon)$ points and has the below guarantee:
    \begin{itemize}
        \item If $M$ is a tree metric, the algorithm outputs \textbf{TREE METRIC} with probability 1;
        \item If $M$ is $\epsilon$-far from any tree metric, the algorithm outputs \textbf{NON-TREE-METRIC} with probability at least 2/3.
    \end{itemize}
    \qed
\end{thm}
\begin{algorithm}
\caption{Tree Metric Testing}\label{algo:tree}
\begin{algorithmic}
\Procedure{TestTreeMetric}{$M$}
\State\Comment{$M\in \mathbb{R}^{n\times n}$ is a distance matrix on $n$ points}
\State $U\gets$ sample $192/\epsilon\cdot \log(48/\epsilon)$ points at random
\For{every four-point-tuple $(u,v,w,z) \in U$}
\If {$TestViolation(M,u,v,w,z)= $ FAIL}
\State\Return \{NON-TREE-METRIC\}
\EndIf
\EndFor
\State $P\gets$ sample $16/\epsilon$ pairs of points at random
\For{every four-point-tuple $(u,v,w,z) \in U\cup P$}
\If {$TestViolation(M,u,v,w,z)=$ FAIL}
\State\Return \{NON-TREE-METRIC\}
\EndIf
\EndFor
\State\Return TREE METRIC

\EndProcedure

\Statex
\Procedure{TestViolation}{M,u,v,w,z}\State\Comment{$u,v,w,z$ are four points in the distance matrix $M$}
\If{$M(u,v)+M(w,z)>\max\{M(u,w)+M(v,z),M(v,w)+M(u,z)\}$ \\or $M(u,w)+M(v,z)>\max\{M(u,v)+M(w,z),M(v,w)+M(u,z)\}$ \\or $M(v,w)+M(u,z)>\max\{M(u,v)+M(w,z),M(u,w)+M(v,z)\}$}
\State\Return FAIL
\EndIf
\State\Return PASS
\EndProcedure
\end{algorithmic}
\end{algorithm}




==> non-important.tex <==
We will first show that, given a weighted clique graph on $n$ vertices, if the weight of $\epsilon n^2$ many edges need to be modified for the clique to satisfy the metric property, then there must be many ``clues of corruptions" showing up in the graph. That is, there are many cycles of short lengths that violate the metric property. We then use these short cycles to find more 3-cycles that violates the triangle inequality. Finally, we show that there are either significantly many unbalanced 3-cycles that Chebyshev's inequality applies even when variance is high, or there are not as many (but still enough) unbalanced edge-disjoint 3-cycles that Chebyshev's inequality applies with low variance. 

First, we define unbalanced cycles and the chords on the cycles. The unbalanced cycles are evidence to the graph violates metric property.
\begin{definition}
    A cycle $c=\{v_1,v_2,...,v_i,v_1\}$ is unbalanced if some edge $(v_j,v_{j+1})\in c$ with weight $w_{(v_j,v_{j+1})}$ larger than the sum of weights of all other edges in $c$. We call this edge $(v_j,v_{j+1})\in c$ the heavy edge of $c$. Otherwise, it is a balanced cycle. For any vertices $v_j,v_k$ on the cycles such that the edge $(v_j,v_k)$ is not on the cycle, we call the edge $(v_j,v_k)$ a chord of this cycle.
\end{definition}
An unbalanced cycle is an evidence of violation of metric property because if all triangles in the graph have weights that obey triangle inequality, then all cycles in the graph are balanced. This is due to iteratively applying the following fact.
\begin{proposition}
    Suppose a cycle $c=\{v_1,v_2,...,v_i,v_1\}$ is unbalanced. Then there exists a chord $(v_j,v_k),j<k,$ such that one of the cycles $c_1=\{v_1,...,v_j,v_k,v_{k+1},...,v_i,v_1\},$ $c_2=\{v_j,v_{j+1},...,v_{k},v_j\}$ is unbalanced. In later analysis, the cycle $c_1$ that contains the heavy edge of $c$ is denoted as $top(c,(v_j,v_k))$ and the other cycle $c_2$ is denoted as $bottom(c,(v_j,v_k))$.
\end{proposition}
\begin{proof}
    Without loss of generality, assume the edge $(v_1,v_2)$ is the heavy edge of cycle $c$. If both cycles $c_1,c_2$ are balanced, then $w_{(v_1,v_2)}$ is at most the sum of weights of all other edges in $c_1$, including $w_{(v_j,v_k)}$, and $w_{(v_j,v_k)}$ is at most the sum of all other edges in $c_2$. Thus, $w_{(v_1,v_2)}$ should be at most the sum of all other edges in $c$ as the union of edges in $c_1,c_2$ minus $(v_j,v_k)$ is exactly the edges in $c$.
\end{proof}

Now, consider the set of all unbalanced triangles. If we remove the set from the graph $G$ completely and obtain $G'$, then there is no unbalanced cycles in $G'$. If $(u,v)$ is in the removal, we define the new weight of $(u,v)$ to be the shortest path from $u$ to $v$ in $G'$. The newly obtained clique is then a metric. This implies that the set of all unbalanced triangles act as a ``fix" to $G$, so the number of edges in the set cannot be smaller than $\epsilon n^2$ given that $G$ is $\epsilon$-far from being a metric. In consequence, there must be at least $\epsilon n^2/3$ unbalanced triangles existing in the graph.

Since the tester samples $\Omega((n/\epsilon^2)^{1/3})$ vertices and make clique-like queries between them, among the $\epsilon n^2/3$ unbalanced triangles, in expectation one of them appears in our sample. However, the variance might be large so we cannot conclude that with high probability there exist an unbalanced triangle in the sample. Such a claim can be made, on the other hand, if all the $\epsilon n^2/3$ unbalanced triangles are edge-disjoint. Hence, we want edge-disjoint unbalanced triangles to appear in $G$ as many as possible.

Let $C^3$ be a maximal set of edge-disjoint triangles in $G$, and let $G^3$ be the graph obtained from removing edges in $C^3$ from $G$. It is not always the case that there is a way to change only edges in $C^3$ to fix $G$ into a metric graph. This is because there might be unbalanced 4-cycles existing in $G^3$, so no matter how edges in $C^3$ are modified, $G^3$ cannot be turned into a metric. Thus, there is no lower bound on the size of $C^3$ at this moment, and as a result, we cannot say much about the number of unbalanced triangles in $C^3$.

Since $G^3$ is not yet a metric, a natural idea is to consider the edge-disjoint unbalanced 4-cycles in $G^3$ and modify them. But new problems emerges: there might be unbalanced 5-cycles or even longer ones after removing the 4-cycles.

A sequence of lemma proved in~\cite{FRB} extends this idea of fixing unbalanced cycles. More importantly, they provide a stopping point so that we do not need to consider indefinitely long unbalanced cycles.
\begin{definition}[unit cycle]For an unbalanced cycle $C$, if there exists a chord $e$ of $C$ such that $bottom(C, e)$ isunbalanced and $e$ is the top edge of $bottom(C, e)$, then $C$ is called a non-unit cycle, otherwise $C$ is called a unit cycle.\end{definition}
\begin{lemma}\label{unitCycleSuffice}
    Suppose $S$ is a set such that, for any unit cycle $c$ in $G$, a non-heavy edge of $c$ is in $S$. then there exists a way of modifying merely edges in $S$ to change $G$ into a metric graph.
\end{lemma}
\begin{proof}
    See Observation 4.1 in~\cite{FRB}.
\end{proof}
\begin{lemma}\label{unbalancedCycleSuffice}
    If set $S$ is a edge cover of all unbalanced
cycles, then $G$ can be converted into a metric graph by only changing weights of edges
in $S$.
\end{lemma}
\begin{proof}
    See Lemma 5.2 in~\cite{FRB}.
\end{proof}
\begin{lemma}\label{unitCycleUnbalance}
    For any chord $e$ of a unit cycle $C$, $top(C, e)$ is unbalanced, with the same
heavy edge as $C$.
\end{lemma}
\begin{proof}
    See Lemma 4.3 in~\cite{FRB}.
\end{proof}
\begin{lemma}\label{length6Cycle}
    Let $S$ be a set such that for any unbalanced unit cycle $c$ of length at most 6, a non-heavy edge of $c$ is in $S$. Then
for any unit cycle $C$ with strictly more than $k$ edges, if the non-heavy edge of $C$ is not in $S$, then for any chord $e$ such that $top(C, e)$ has at most 6 edges, $e\in S$.
\end{lemma}
\begin{proof}
    See Corollary 4.5 in~\cite{FRB}.
\end{proof}

Now we have enough tools to proceed. Continue the previous procedure of creating $C^3$, let $C^4$ be a maximal set of edge-disjoint unit 4-cycles in $G^3$, and remove edges in $C^4$ from $G^3$ to get a graph $G^4$. Likewise, define maximal edge-disjoint unit unbalanced cycle sets $C^5,C^6$ and the remainder graphs $G^5,G^6$. Now, follow the procedure below to get the last set $C^{t4}$ and remainder graph $G^{t4}$.
\begin{enumerate}
    \item Initiate $G^{t4}=G^6$ and $C^{t4}=\emptyset$.
    \item If there exists a unit unbalanced cycle $c$ of length $>6$ in $G^{t4}$ of the form $c=\{v_1,v_2,v_3...,v_i,v_1\}$ where $(v_1,v_2)$ is the heavy edge, add the 4-cycle $\{v_1,v_2,v_3,v_i,v_1\}$ into $C^{4t}$, and remove edges $(v_1,v_2),(v_2,v_3),(v_i,v_1)$ from $G^{t4}$. Note that the edge $(v_3,v_i)$ might overlap with other edges in $C^3,C^4,C^5,C^6,C^{4t}$. Hence, denote this special edge as $opposite(c)$, as it is at the opposite side from the heavy edge of $c$.
    \item Repeat step 2 until there is no unit unbalanced cycle of length $>6$ in $G^{t4}.$
\end{enumerate}
Note that, except for the $opposite(c)$ edges, the set of cycles $C^3,C^4,C^5,C^6,C^{4t}$ are edge-disjoint. Moreover, we claim that $G$ can be fixed into a metric graph by only changing weights in $C^3\cup C^4\cup C^5\cup C^6\cup C^{4t}$.
\begin{proposition}
    $G$ can be fixed into a metric graph by only changing weights in $C^3\cup C^4\cup C^5\cup C^6\cup C^{4t}$.
\end{proposition}
\begin{proof}
    By \hyperref[unbalancedCycleSuffice]{Lemma~\ref*{unbalancedCycleSuffice}}, we only need to show that any unbalanced cycle $c\in G$ has an edge in the union. By construction, if $c$ is an unit cycle with length $i\leq6$, at least one of its edges is added into $C^3\cup C^4\cup C^5\cup C^6$. If $c$ is an unit cycle with length $i>6$ and if none of its edges is in $C^3\cup C^4\cup C^5\cup C^6$, then at least one of its edges is added to $C^{4t}$.

    On the other hand, for non-unit cycles, there must exists a chord $e$ such that $bottom(c,e)$ is unbalanced with $e$ as its heavy edge. Take the smallest such $bottom(c,e)$ and it must be an unit unbalanced cycle $c'$. The heavy edge of $c'$ is $e$ and the two edges incident to $e$ in $c'$ are also in $c$. Moreover, by construction, these two edges along with $e$ are in the union. Thus, some edge of $c$ is in the union. 
\end{proof}

The above result shows that the union $C^3\cup C^4\cup C^5\cup C^6\cup C^{4t}$ is a valid fix for the graph $G$, so the number of edges $|C^3\cup C^4\cup C^5\cup C^6\cup C^{4t}|$ is at least $\epsilon n^2$. This indicates that one of the five sets of cycles $C^i$ has more than $\epsilon n^2/5$ edges, so more than $\epsilon n^2/30$ cycles.

We are perfectly content if this set is $C^3$, because with this large set of edge-disjoint triangles, a random sampling hits some unbalanced triangles with high probability. But it could be the case that $C^3$ is small. Still, we will show that one of $C^4,C^5,C^6,C^{4t}$ being large also creates good structual property. Before moving forward, we make some modifications to the cycles in $C^4,C^5,C^6$ so that they emulate the cycles in $c^{4t}$. In this way we can analyze the four sets with generality.

For each cycle $c\in C^4,C^5,C^6$, suppose c is of the form $\{v_1,v_2,v_3,...,v_i,v_1\}$ and edge $(v_1,v_2)$ is the heavy edge of $c$. We replace the cycle $c$ with a new cycle $c'=\{v_1,v_2,v_3,v_i,v_1\}$. That is, we keep the heavy edge $(v_1,v_2)$, the two edges $(v_2,v_3),(v_i,v_1)$ incident to it, and add the chord $(v_3,v_i)$. Denote this newly added edge $(v_3,v_i)$ the $opposite(c')$ and denote the three old edges $originals(c')$. Notice that it is no longer the case that all cycles in $C^4,C^5,C^6$ are edge-disjoint because they could share the same $opposite(c)$ edge, and $opposite(c)$ might be one of $originals(c')$ for some cycles $c,c'$. By \hyperref[unitCycleUnbalance]{Lemma~\ref*{unitCycleUnbalance}}, after this replacement, every cycle in $C^4,C^5,C^6$ remains to be unbalanced. At this point, four cycle sets $C^4,C^5,C^6,C^{4t}$ all satisfy the below properties.

\begin{enumerate}
    \item $C^i$ only contains 4-cycles.
    \item Any cycle $c\in C^i$ is unbalanced.
    \item The heavy edge of $c$ forms two triangles with two chords of $c$, respectively. By \hyperref[unitCycleUnbalance]{Lemma~\ref*{unitCycleUnbalance}}, the two triangles are also unbalanced. (We don't need the chords to be in $C^i$.)
    \item For two cycles $c_1,c_2\in C^i$, the six edges in $originals(c_1)\cup originals(c_2)$ are different. If $c_1,c_2$ share some edge, it could only be one of the cases
    \begin{enumerate}
        \item $opposite(c_1)=opposite(c_2)$
        \item $opposite(c_1)\in originals(c_2)$
        \item $opposite(c_2)\in originals(c_1)$
    \end{enumerate}
\end{enumerate}

From now on, let $C$ be some $C^4,C^5,C^6,C^{4t}$ with at least $\epsilon n^2/30$ cycles. Now we get to the core and the most intricate part of the analysis: use cycles in $C$ to create a large amount of unbalanced triangles. The third property hints at how we are going to find the unbalanced triangles. Thus, we take a closer look at the chords of cycles in $C$.

Notice that each cycle in $C$ has exactly two chords. Let $R$ be the set of chords in $C$. We create a graph $CHORDS=(V^{chords},E^{chords})$ based on the chords relations in $C$. Let the vertex set $V^{chords}$ of $CHORDS$ be the set of different chords in $C$. Thus, the edges in $CHORDS$ corresponds to the cycles in $C$: if a cycle $c$ has two chords $e_1,e_2$, then the corresponding two vertices in $CHORDS$ are connected by an edge. That is, create a bijective mapping $\phi:R\rightarrow V^{chords}$ and define edges $(\phi(e_1),\phi(e_2))\in E^{chords}$ if $\exists c\in C$, $e_1,e_2$ are two chords of $c$. Thus, we naturally could extend the mapping $\phi$ to another mapping $\phi':C\rightarrow E^{chords},$ where for some cycle $c=\{v_1,v_2,v_3,v_4,v_1\}\in C$, $\phi'(c)=(\phi(v_1,v_3),\phi(v_2,v_4))\in E^{chords}$. To simplify the notation, we alternatively use $(v_1,v_2,v_3,v_4)$ to denote the same cycle as $\{v_1,v_2,v_3,v_4,v_1\}$.

The gist for the following analysis is either $|V^{chords}|$ is large enough and we could obtain a large set of edge-disjoint triangles, or $|V^{chords}|$ is small, meaning many cycles in $C$ have to share common chords, which engenders a significant amount of unbalanced triangles. Formally, the relationship between $|V^{chords}|$ and the number of edge-disjoint triangles is shown below.
\begin{proposition}
    There exists a set of $|V^{chords}|/8$ edge-disjoint unbalanced triangles.
\end{proposition}
\begin{proof}
    We propose below a procedure of finding a set of edge-disjoint unbalanced triangles based on the graph $CHORDS$.

    Previously, we mentioned that each cycle in $C$ produces two unbalanced triangles. We will first prune this set of triangles so that any two triangles have different chord-edge. Then, we further prune the set to make the triangles edge-disjoint.

    We first find a spanning forest for $CHORDS$. Notice that there is no isolated vertex in $CHORDS$, so any spanning tree in the spanning forest contains at least 2 vertices. Initialize an empty set $T$, which later will contain all the desired triangles. Focus on a spanning tree: starting from any leaf $\phi((u,v))\in V^{chords}$ (corresponding to a chord $(u,v)$) and its incident edge $\phi'((u,w,v,z))\in E^{chords}$ (corresponding to a cycle $(u,w,v,z)\in C$ having $(u,v)$ as one of its chords), add the unbalanced triangle corresponding to the chord-cycle pair to the set $T$. That is, the unbalanced triangle $(u,v,w)$ or $(u,v,z)$ inside the cycle $(u,w,v,z)$ using the chord $(u,v)$. (Recall that for any chord in the cycle $(u,w,v,z),$ the triangle formed by the chord and the heavy edge of $(u,w,v,z)$ must be unbalanced. Hence one of $(u,v,w)$ or $(u,v,z)$ must be unbalanced.) After adding the unbalanced triangle corresponding to one leaf and its incident edge, remove the leaf and the incident edge from the spanning tree. Repeat adding triangles and removing (leaf, incident edge) pair until the spanning tree only has one vertex left, and we move on to the next spanning tree.

    Since each spanning tree initially has at least two vertices and the spanning forest has $|V^{chords}|$ many vertices, we eventually added at least $|V^{chords}|/2$ many triangles to $T$.

    Moreover, each triangle added to $T$ has a ``chord-edge" and two ``cycle-edges", where ``chord-edge" corresponds to the leaf and the ``cycle-edges" are edges in the cycle corresponding to the incident edge of the leaf. For two triangles in $T$, they have different chord-edges and the four cycle-edges are also different.

    However, two triangles $t_1,t_2$ in $T$ can still have an overlapping edge. This can happen if the chord-edge of $t_1$ is one of the cycle-edges of $t_2$, or oppositely. Now, we create a helper graph where each node represents a triangle in $T$. One node $t_1$ has an out-edge pointing to node $t_2$ if the chord-edge of $t_1$ is one of the cycle-edges of $t_2$. It is straightforward to check that for each node in the graph, the in-degree is at most 2 and the out-degree is at most 1. If we view the helper graph as an undirected graph, the max degree is 3 so the average degree is at most 3. Thus, by Caro-Wei Theorem, there exists an independent set of size at least $|T|/(deg_{avg}+1)\geq |T|/4\geq |V^{chords}|/8$. This independent set corresponds to a subset of $T$ where the triangles are edge-disjoint.
\end{proof}

This result shows that we are in a good shape if $|V^{chords}|$ is large. Hence, we need to consider what will happen if $|V^{chords}|$ is small. The number of different chords in $C$ is small implies that many unbalanced cycles are sharing the same chord. The next proposition shows that whenever two unbalanced cycles share the same chord, they produces an unbalanced triangle.

\begin{proposition}
    Suppose two unbalanced cycles $c_1,c_2\in C$ share the same chord. Then there exists an unbalanced triangle which uses one edge from $c_1$ and one edge from $c_2$. Moreover, these two edges cannot be $opposite(c_1),opposite(c_2)$ at the same time.
\end{proposition}
\begin{proof}
    
\end{proof}









